Thompson Sampling for Combinatorial Semi-bandits with Sleeping Arms and Long-Term Fairness Constraints

We study the combinatorial sleeping multi-armed semi-bandit problem with long-term fairness constraints~(CSMAB-F). To address the problem, we adopt Thompson Sampling~(TS) to maximize the total rewards and use virtual queue techniques to handle the fairness constraints, and design an algorithm called \emph{TS with beta priors and Bernoulli likelihoods for CSMAB-F~(TSCSF-B)}. Further, we prove TSCSF-B can satisfy the fairness constraints, and the time-averaged regret is upper bounded by $\frac{N}{2\eta} + O\left(\frac{\sqrt{mNT\ln T}}{T}\right)$, where $N$ is the total number of arms, $m$ is the maximum number of arms that can be pulled simultaneously in each round~(the cardinality constraint) and $\eta$ is the parameter trading off fairness for rewards. By relaxing the fairness constraints (i.e., let $\eta \rightarrow \infty$), the bound boils down to the first problem-independent bound of TS algorithms for combinatorial sleeping multi-armed semi-bandit problems. Finally, we perform numerical experiments and use a high-rating movie recommendation application to show the effectiveness and efficiency of the proposed algorithm.

==> 6-Proof.tex <==
\section{Proof of Regret Bounds}
%In this section, we prove Theorem \ref{thm:regret} and Theorem \ref{thm:regret2}. The proofs of Theorem \ref{thm:regret} and Theorem \ref{thm:regret2} are similar but they use different concentration inequalities in the end of the analysis.
\subsection{Notations}
Recall $\hat{u}_{i}(t) := \frac{\alpha_{i}(t)-1}{h_{i}(t)}=\frac{1}{h_{i}(t)} \sum\limits_{\tau: \tau<t, i \in A(\tau)} X_{i}(t)$ is the empirical mean of arm $i$ until the beginning of round $t$.  Therefore, we have $\alpha_i(t) -1  = \hat{u}_{i}(t) h_i(t) = \hat{u}_{i}(t) (\alpha_{i}(t) + \beta_i(t)-2)$. 

For each arm $i\in \mathcal{N}$, we have three events $\mathcal{J}_i(t)$, $\mathcal{K}_i(t)$ and $\mathcal{H}_i(t)$ defined as follows:
\begin{equation*}
\begin{aligned}
   &\mathcal{J}_i(t) := \{\theta_i(t)  - u_i > 2\gamma_i(t) \},\\
   &\mathcal{K}_i(t) := \{u_i - \theta_i(t)> 2\varepsilon_i(t) \},\\
   &\mathcal{K}_i(t) := \{u_i - \theta_i(t)> 2\gamma_i(t).
\end{aligned}
\end{equation*}
where $\gamma_i(t) := \sqrt{\frac{2\ln T}{h_i(t)}}, \varepsilon_i(t) := \sqrt{\frac{2\ln t}{h_i(t)}}$. 


\subsection{Proof of Theorem \ref{thm:regret}}\label{sec:thm52}
To prove Theorem \ref{thm:regret}, we first introduce the following lemmas with the proofs in Sec.~\ref{sec:pfoflemmas}.

\begin{lemma}\label{lm:main}
\cite{li2019combinatorial}. Then the time-average regret of TSCSF-B or TSCSF-G can be bounded by
\begin{equation}\label{eq:astar}
\small
\begin{aligned}
\frac{N}{2 \eta}+\frac{1}{T} \left(\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i \in A(t)} w_{i}\left(\theta_{i}(t)-u_{i}\right)\right]}_{C_1} +  \underbrace{\sum_{t=0}^{T-1}\mathbb{E}\left[\sum_{i \in A^{\prime}(t)} w_{i}\left(u_{i}-\theta_{i}(t)\right)\right]}_{C_2}\right).
\end{aligned}
\end{equation}
\end{lemma}



\begin{lemma}\label{lm:ft}
For all $i \in \mathcal{N}, t \leq T$, the probability that event ${\mathcal{J}_i(t)}$ happens is upper bounded as follows:
\begin{equation*}
    \Pr\left(\mathcal{J}_i(t)\right) \leq \frac{1}{T} + \frac{1}{T^4},
\end{equation*}
\end{lemma}

\begin{lemma}\label{lm:kt}
For all $i \in \mathcal{N}, h_i(t) \geq 4$ and $t \leq T$, the probability that event ${\mathcal{K}_i(t)}$ happens is upper bounded as follows:
\begin{equation*}
    \Pr\left(\mathcal{K}_i(t)\right) \leq \frac{1}{t^2} + \frac{1}{t^4}.
\end{equation*}
\end{lemma}

\begin{proof}
First, by Lemma \ref{lm:main} we have $R_{\mathrm{TSCSF-B}}(T)$ bounded by
(\ref{eq:astar}).

\paragraph{Bound $C_1$}
Define event $\overline{\mathcal{J}_i(t)}$ is the complementary event of $\mathcal{J}_i(t)$ as follows:
\begin{equation*}
    \overline{\mathcal{J}_i(t)} := \{\theta_i(t) - u_i \leq 2\gamma_i(t) \}.
\end{equation*}
Then, we can decompose $C_1$ as
\begin{equation*}\label{eq:c1}
\begin{aligned}
    &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}[\mathcal{J}_i(t)] \right]}_{B_1} \\
    + &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}[\overline{\mathcal{J}_i(t)}] \right]}_{B_2}.
\end{aligned}
\end{equation*}
Since $\theta_{i}(t)-u_{i}\leq 1, d_{i}(t)\leq 1$, $B_1$ is therefore bounded by
\begin{equation*}\label{eq:b2}
\begin{aligned}
    \sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i} \mathbf{1}[{\mathcal{J}_i(t)}] \right] \leq & w_{\max}\sum_{i=1}^{N} \sum_{t=0}^{T-1} \Pr\left({\mathcal{J}_i(t)}\right)\\
    \leq & w_{\max}\sum_{i=1}^{N} \sum_{t=0}^{T-1} \left(\frac{1}{T}+\frac{1}{T^4}\right)\\
    \leq & 2 w_{\max} N,
\end{aligned}
\end{equation*}
where the second inequality is due to Lemma \ref{lm:ft}.


Next, we show how to bound $B_2$. Let $\tau_{i}(a)$ be the round where arm $i$ is played for the $a$-th time, i.e., $h_{i}(\tau_{i}(a)) = a-1$.
$B_2$ can be bounded as follows:
\begin{equation}\label{eq:B1}
\begin{aligned}
    &\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}\left[\overline{\mathcal{J}_i(t)}\right] \right]\\
    =&\sum_{i=1}^{N} \mathbb{E}\left[\sum_{a=1}^{h_{i}(T-1)} \sum_{\tau_i(a)}^{\tau_{i}(a+1)-1} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}\left[\overline{\mathcal{J}_i(t)}\right]\right]\\
    \leq& \sum_{i=1}^{N} \mathbb{E}\left[w_{1} + \sum_{a=2}^{h_{i}(T-1)} \sum_{\tau_i(a)}^{\tau_{i}(a+1)-1} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}\left[\overline{\mathcal{J}_i(t)}\right]\right]\\
    \leq& w_{\max}\sum_{i=1}^{N} \mathbb{E}\left[1 + 2 \sum_{a=2}^{h_{i}(T-1)} \sum_{\tau_i(a)}^{\tau_{i}(a+1)-1} \gamma_i(t) d_{i}(t) \right]\\
    =& w_{\max}N + 2w_{\max}\sum_{i=1}^{N} \mathbb{E}\left[\sum_{a=2}^{h_{i}(T-1)} \gamma_i(\tau_i(a))\right].
\end{aligned}
\end{equation}
The last term in (\ref{eq:B1}) can be further written as follows:
\begin{equation*}\label{eq:2wb}
    \begin{aligned}
    & 2w_{\max}\sum_{i=1}^{N}  \mathbb{E}\left[ \sum_{a = 2}^{h_i(T-1)} \gamma_i(\tau_i(a))\right]\\ 
    =& 2w_{\max}\sum_{i=1}^{N} \mathbb{E}\left[ \sum_{a = 2}^{h_i(T-1)} \sqrt{\frac{2\ln T}{a-1}}\right]\\
    =& 2w_{\max} \sqrt{2\ln T} \sum_{i=1}^{N}  \mathbb{E}\left[ \sum_{a = 2}^{h_i(T-1)} \sqrt{\frac{1}{a-1}}\right] \\
    {\leq} & 2w_{\max} \sqrt{2\ln T} \sum_{i=1}^{N}  \mathbb{E}\left[ 1 + \int_{1}^{h_i(T-1)} \sqrt{\frac{1}{x}} dx \right]\\
     {\leq}& 2w_{\max} \sqrt{2\ln T} \sum_{i=1}^{N}  \mathbb{E}\left[ \sqrt{h_i(T-1)}\right]\\
     {\leq} & 2w_{\max} \sqrt{2\ln T} \sum_{i=1}^{N}   \sqrt{\mathbb{E}\left[h_i(T-1)\right]},
    \end{aligned}
\end{equation*}
where the last inequality is due to Jensen's inequality. Also by Jensen's inequality, we have
\begin{equation*}
    \frac{1}{N}\sum\limits_{i=1}^{N}   \sqrt{\mathbb{E}\left[h_i(T-1)\right]} \leq \sqrt{\frac{1}{N} \sum\limits_{i=1}^{N}\mathbb{E}\left[h_i(T-1)\right]}.
\end{equation*}
Therefore, we can bound $\sum\limits_{i=1}^{N}   \sqrt{\mathbb{E}\left[h_i(T-1)\right]}$ by
\begin{equation*}\label{eq:lb1t}
\begin{aligned}
     \sqrt{N \sum\limits_{i=1}^{N}\mathbb{E}\left[h_i(T-1)\right]}
    \leq \sqrt{NTm},
\end{aligned}
\end{equation*}
where the inequality is due to the fact that at most $m$ arms are selected in each round.
Therefore, we have $B_2$ bounded by
\begin{equation*}\label{eq"b1bound}
    2w_{\max} \sqrt{2mNT\ln T} + w_{\max}N.
\end{equation*}


Combining $B_1$ and $B_2$ gives
\begin{equation*}
    C_1 \leq 2w_{\max}\sqrt{2mNT\ln T} +  3w_{\max}N.
\end{equation*}

\paragraph{Bound $C_2$} 
Define an event $\overline{\mathcal{K}_i(t)}$ as the complementary event of $\mathcal{K}_i(t)$:
\begin{equation*}
    \overline{\mathcal{K}_i(t)} := \{u_i - \theta_i(t) \leq 2\varepsilon_i(t)\}.
\end{equation*}
$C_2$ can be decomposed by
\begin{equation*}\label{eq:c2}
\begin{aligned}
    &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d^\prime_{i}(t) \mathbf{1}\left[\mathcal{K}_i(t)\right]\right]}_{B_3} \\
    + &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d^\prime_{i}(t) \mathbf{1}\left[\overline{\mathcal{K}_i(t)}\right] \right]}_{B_4}.
\end{aligned}
\end{equation*}

Let $\tau^\prime_{i}(a)$ be the round where arm $i$ is played for the $a$-th time by policy $A^\prime(t)$, i.e., $h^\prime_{i}(\tau^\prime_{i}(a)) = a - 1$. Since $\theta_{i}(t)-u_{i}\leq 1$, we can write $B_3$ as follows:
\begin{equation*}\label{eq:b4}
\begin{aligned}
    B_4 \leq& w_{\max} \sum_{i=1}^N \mathbb{E}\left[\sum_{t=1}^{T-1} d^\prime_{i}(t) \mathbf{1}\left[\overline{\mathcal{K}_i(t)}\right] \right] \\
    =& w_{\max} \sum_{i=1}^N \mathbb{E}\left[\sum_{a=1}^{h_i^\prime(T-1)} \mathbf{1}\left[\overline{\mathcal{K}_i(\tau^\prime_{i}(a))}\right] \right] \\
    \leq & w_{\max} \sum_{i=1}^N \mathbb{E}\left[\sum_{a=1}^{3}1 + \sum_{a=4}^{h_i^\prime(T-1)} \mathbf{1}\left[\overline{\mathcal{K}_i(\tau^\prime_{i}(a))}\right] \right]\\
    \leq & 3w_{\max}N +  w_{\max} \sum_{i=1}^N \sum_{a=4}^{\infty} \Pr\left(\overline{\mathcal{K}_i(\tau^\prime_{i}(a))}\right)\\
    \stackrel{(\rm a)}{=} & 3 w_{\max} N + w_{\max} \sum_{i=1}^N \sum_{a=4}^{\infty} \left(\frac{1}{(\tau^\prime_{i}(a))^2} + \frac{1}{(\tau^\prime_{i}(a))^4} \right)\\
    \leq & 3 w_{\max} N + w_{\max} \sum_{i=1}^N \sum_{t=1}^{\infty} \left(\frac{1}{t^2} + \frac{1}{t^4} \right)\\
    \leq & 3 w_{\max} N + w_{\max} \sum_{i=1}^N  \left(\frac{\pi^2}{6} + \frac{\pi^4}{90} \right)\\
    \leq & 5.73w_{\max}N.
\end{aligned}
\end{equation*}
where (a) is due to Lemma \ref{lm:kt}.

$B_4$ can be bounded in a similar way as $B_2$:
\begin{equation*}\label{eq:b3}
\begin{aligned}
    B_3 \leq& w_{\max}N + 2w_{\max} \sum_{i=1}^{N} \mathbb{E}\left[\sum_{a=2}^{h^\prime_i(T-1)}\sqrt{\frac{2 \ln t}{a-1}} \right]\\
    \leq & w_{\max}N  + 2w_{\max} \sqrt{\ln T} \sum_{i=1}^{N} \mathbb{E}\left[\sum_{a=2}^{h^\prime_i(T-1)}\sqrt{\frac{1}{a-1}} \right]\\
    \leq & 2w_{\max} \sqrt{2mNT\ln T} + w_{\max}N .
\end{aligned}
\end{equation*}

Therefore, we have $C_2$ bounded by
\begin{equation*}\label{eq:c21}
    2w_{\max}\sqrt{2mNT\ln T} + 6.73 w_{\max}N.
\end{equation*}
Theorem \ref{thm:regret} is proved by combining the bound of $C_1$ and $C_2$.
\end{proof}

\subsection{Proof of Theorem \ref{thm:regret2}}\label{pf:regret2}
To bound Theorem \ref{thm:regret2}, we introduce the following Lemma with a proof in Sec.~\ref{sec:pfoflemmas}:
\begin{lemma}\label{lm:gs}
For all $i \in \mathcal{N}, h_i(t)>0$ and $t \leq T$, the probabilities that event ${\mathcal{J}_i(t)}$ happens and event ${\mathcal{H}_i(t)}$ happens are upper bounded as follows:
\begin{equation*}
\begin{aligned}
    &\Pr\left({\mathcal{J}_i(t)}\right) \leq \frac{1}{2T} + \frac{1}{T^4},\\
    &\Pr\left({\mathcal{H}_i(t)}\right) \leq \frac{1}{2T} + \frac{1}{T^4}.
\end{aligned}
\end{equation*}
\end{lemma}

\begin{proof}
Similar to the proof of Theorem \ref{thm:regret}, we first use Lemma \ref{lm:main} to have $R_{\mathrm{TSCSF-G}}(T)$ bounded by
\begin{equation}
\begin{aligned}
\frac{N}{2 \eta}+\frac{1}{T} \left(C_1 + C_2\right).
\end{aligned}
\end{equation}

Then we can decompose $C_1$ as follows:
\begin{equation}\label{eq:c3}
\begin{aligned}
    &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}[\mathcal{J}_i(t)] \right]}_{B_5} \\
    + &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}[\overline{\mathcal{J}_i(t)}] \right]}_{B_6}.
\end{aligned}
\end{equation}
We can bound $B_5$ by Lemma \ref{lm:gs} as follows:
\begin{equation}\label{eq:b6}
\begin{aligned}
    B_6 \leq& w_{\max} \sum_{i=1}^{N} \mathbb{E}\left[\sum_{t=0}^{T-1} \mathbf{1}[{{\mathcal{J}_i(t)}}] \right]\\
    =& w_{\max} \sum_{i=1}^{N} \sum_{t=0}^{T-1} \Pr\left({{\mathcal{J}_i(t)}}\right)\\
    \leq& w_{\max} \sum_{i=1}^{N} \sum_{t=0}^{T-1} \left(\frac{1}{2T}+\frac{1}{T^4}\right)\\
    \leq& 1.5 w_{\max} N.
\end{aligned}
\end{equation}


On the other hand, we can bound $B_6$ in the same way as $B_2$ by
\begin{equation}\label{eq:b5}
    2w_{\max} \sqrt{2mNT\ln T} + w_{\max}N.
\end{equation}


Substituting (\ref{eq:b6}) and (\ref{eq:b5}) into (\ref{eq:c3}), we have $C_1$ bounded by
\begin{equation*}
    2w_{\max}\sqrt{2mNT\ln T} + 2.5 w_{\max} N.
\end{equation*}

Define event $\overline{\mathcal{H}_i(t)}$ as the complementary event of $\mathcal{H}_i(t)$:
\begin{equation*}
    \overline{\mathcal{H}_i(t)} = \{\theta_i(t)-u_i\leq 2\gamma_i(t) \}.
\end{equation*}

$C_2$ can be decomposed by whether events $\mathcal{H}_i(t)$ and $\overline{\mathcal{H}_i(t)}$ happen as follows:

\begin{equation*}\label{eq:c2}
\begin{aligned}
    &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d^\prime_{i}(t) \mathbf{1}\left[\mathcal{H}_i(t)\right]\right]}_{B_7} \\
    + &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d^\prime_{i}(t) \mathbf{1}\left[\overline{\mathcal{H}_i(t)}\right] \right]}_{B_8}.
\end{aligned}
\end{equation*}

We have $B_7$ bounded by $1.5w_{\max}N$ with Lemma \ref{lm:gs}, and $B_8$ bounded by $2w_{\max}\sqrt{2mNT\ln T} + 2.5 w_{\max} N$ with the same steps as bounding $B_1$.
Theorem \ref{thm:regret2} is proved by combining $C_1$ and $C_2$ together.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%proof of lemmas%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemmas}\label{sec:pfoflemmas}

\subsubsection{Proof of Lemma \ref{lm:main}}

\begin{proof}
The proof for Lemma \ref{lm:main} is similar to Theorem 1 in~\cite{li2019combinatorial}. 

Note that the arms selection (defined in (\ref{eq:solution})) is different from LFG~\cite{li2019combinatorial}(we put $\eta$ with the virtual queue), we show that Lemma \ref{lm:main} works for our setting as well.

Following the similar lines in \cite{li2019combinatorial,neely2010stochastic}, we first consider the Lyapunov drift function:
\begin{equation*}
    L(\mathbf{Q}(t)) := \frac{1}{2} \sum_{i=1}^{N} Q_{i}^{2}(t).
\end{equation*}
Recall the regret definition as follows:
\begin{equation*}
\begin{aligned}
    \mathcal{R}(T) &:= \mathbb{E}\left[\frac{1}{T} \sum_{t=0}^{T-1} {\left(\sum_{i \in A^*(t)} w_{i} X_{i}(t) - \sum_{i \in A(t)} w_{i} X_{i}(t)\right)}\right]\\
    & = \frac{1}{T} \sum_{t=0}^{T-1}\mathbb{E}\left[\sum_{i \in A^*(t)} w_{i} u_{i}(t) - \sum_{i \in A(t)} w_{i} u_{i}(t)\right]\\
    & = \frac{1}{T} \sum_{t=0}^{T-1}\mathbb{E}\left[\underbrace{\sum_{i = 1}^N w_{i} u_{i}(t) d^*_i(t)- \sum_{i = 1}^N w_{i} u_{i}(t) d_i(t)}_{\Delta r_i(t)} \right].,
\end{aligned}
\end{equation*}
where $d^*_i(t) = \mathbf{1}\left[i \in A^*_i(t) \right]$ and $d_i(t) = \mathbf{1}\left[i \in A_i(t) \right]$.

Then, the drift-plus-regret is given by
\begin{equation}
\begin{aligned}
    &L(\mathbf{Q}(t+1))-L(\mathbf{Q}(t))+\eta \Delta r_i(t) \\ 
    &=\frac{1}{2} \sum\limits_{i=1}^{N} Q_{i}^{2}(t+1)-\frac{1}{2} \sum\limits_{i=1}^{N} Q_{i}^{2}(t)+\eta \Delta r_i(t) \\ 
    &\stackrel{(\rm a)} {=}\frac{1}{2}\sum\limits_{i=1}^{N}\left(Q_{i}(t)+k_{i}-d_{i}(t)\right)^{2}-\frac{1}{2} \sum\limits_{i=1}^{N} Q_{i}^{2}(t)+\eta \Delta r_i(t) \\ 
    &=\frac{1}{2} \sum\limits_{i=1}^{N}\left(k_{i}-d_{i}(t)\right)^{2}+\sum\limits_{i=1}^{N}\left(k_{i}-d_{i}(t)\right) Q_{i}(t)+\eta \Delta r_i(t) \\ 
    &\stackrel{(\rm b)} {\leq} \frac{N}{2}+\sum\limits_{i=1}^{N} k_{i} Q_{i}(t)-\sum\limits_{i=1}^{N} d_{i}(t) Q_{i}(t)\\
    &+\eta \sum\limits_{i=1}^{N} w_{i} u_{i} d_{i}^{*}(t)-\eta \sum\limits_{i=1}^{N} w_{i} u_{i} d_{i}(t) \\
    &= \frac{N}{2}+\sum\limits_{i=1}^{N}\left(Q_{i}(t)+\eta w_{i} u_{i}\right)\left(d_{i}^{*}(t)-d_{i}(t)\right) \\ 
    &+\sum\limits_{i=1}^{N} Q_{i}(t)\left(k_{i}-d_{i}^{*}(t)\right),
\end{aligned}
\end{equation}
where (a) is due to (\ref{eq:updateQ}), and (b) is due to facts that $k_{i}-d_{i}(t)\leq 1$ and $\Delta r_i(t) > 0$


We can bound the expected drift-plus-regret as
\begin{equation}\label{eq:dpr}
\begin{aligned}
     &\mathbb{E}[L(\mathbf{Q}(t+1))-L(\mathbf{Q}(t))+\eta \Delta r_i(t)]\\ 
     &\leq \frac{N}{2}+\sum\limits_{i=1}^{N} \mathbb{E}\left[\left(Q_{i}(t)+\eta w_{i} u_{i}\right)\left(d_{i}^{*}(t)-d_{i}(t)\right)\right]\\
     &+\sum\limits_{i=1}^{N} \mathbb{E}\left[Q_{i}(t)\left(k_{i}-d_{i}^{*}(t)\right)\right] \\ 
     &\leq \frac{N}{2}+\mathbb{E}[\sum\limits_{i=1}^{N}\left(Q_{i}(t)+\eta w_{i} u_{i}\right)\left(d_{i}^{*}(t)-d_{i}(t)\right)],
\end{aligned}
\end{equation}
where the last inequality is due to $\mathbb{E}\left[d_{i}^{*}(t)\right] \geq k_{i}$.



Summing (\ref{eq:dpr}) for all
$t\in\{0,\ldots,T-1\}$, and
dividing both sides of the inequality by $T\eta$, we have
\begin{equation*}
\begin{aligned}
    &\frac{1}{T \eta} \mathbb{E}[L(\mathbf{Q}(T))-L(\mathbf{Q}(0))]+\frac{1}{T} \sum\limits_{t=0}^{T-1} \mathbb{E}[\Delta r_i(t)] \\ 
    &\leq \frac{N}{2 \eta}+\frac{1}{T} \mathbb{E}[\underbrace{\sum\limits_{i=1}^{N}  \left(\frac{1}{\eta}Q_{i}(t)+ w_{i} u_{i}\right)\left(d_{i}^{*}(t)-d_{i}(t)\right)}_{C(t)}]
\end{aligned}
\end{equation*}

Since $L(Q(T)) \geq 0$ and $L(Q(0)) = 0$, we have 
\begin{equation}\label{eq:regretbound}
    \mathcal{R}(T) = \frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E}[\Delta r_i(t)] \leq \frac{N}{2 \eta}+\frac{1}{\eta T} \sum_{t=0}^{T-1} \mathbb{E}\left[C(t)\right]
\end{equation}



Recall that in each round $t$, the TSCSF-B and TSCSF-G algorithms choose
arms $A(t)$ according to the follows:
\begin{equation*}
    A(t) \in \underset{A \subseteq {Z}(t), |A| \leq m}{\operatorname{argmax}} \sum_{i \in S}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} \theta_{i}(t)\right),
\end{equation*}
and the oracle (see the sketch proof for Theorem \ref{skpf:regret1}) chooses arms $A^\prime (t)$ as follows:
\begin{equation}\label{eq:1eeeeee}
    A^{\prime}(t) \in \underset{A \subseteq Z(t), |A| \leq m}{\operatorname{argmax}} \sum_{i \in A}\left(\frac{1}{\eta}Q_{i}(t)+w_{i} u_{i}(t)\right).
\end{equation}

Therefore, we have
\begin{equation}\label{eq:1eee}
    \sum_{i \in A(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} \theta_{i}(t)\right) \geq \sum_{i \in A^{\prime}(t)}\left(\frac{1}{\eta} Q_{i}(t) + w_{i} \theta_{i}(t)\right)
\end{equation}

$C(t)$ can be bounded as follows:
\begin{equation}\label{eq:ct}
    \begin{aligned}
    C(t)=& \sum_{i=1}^{N}\left(\frac{1}{\eta} Q_{i}(t)+ w_{i} u_{i}\right)\left(d_{i}^{*}(t)-d_{i}(t)\right) \\
    =& \sum_{i \in A^{*}(t)}\left(\frac{1}{\eta} Q_{i}(t)+ w_{i} u_{i}\right)-\sum_{i \in A(t)}\left(\frac{1}{\eta} Q_{i}(t)+w_{i} u_{i}\right) \\ 
     \stackrel{(\rm a)}{\leq} & \sum_{i \in A^{\prime}(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} u_{i}\right)-\sum_{i \in A(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} u_{i}\right) \\ 
     \stackrel{(\rm b)}\leq & \sum_{i \in A^{\prime}(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} u_{i}\right)-\sum_{i \in A(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} u_{i}\right) \\ 
     +&\sum_{i \in A(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} \theta_{i}(t)\right) -\sum_{i \in A^{\prime}(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} \theta_{i}(t)\right) \\
     =& {\sum_{i \in A(t)} w_{i}\left(\theta_{i}(t)-u_{i}\right)} + {\sum_{i \in A^{\prime}(t)} w_{i}\left(u_{i}-\theta_{i}(t)\right)},
     \end{aligned}
\end{equation}
where (a) is due to the definition of $A^\prime(t)$ in (\ref{eq:1eeeeee}) and (b) is due to (\ref{eq:1eee}).

Substituting (\ref{eq:ct}) into (\ref{eq:regretbound}) concludes the proof.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma  \ref{lm:ft}}
\begin{proof}
Let event $\mathcal{A}_i(t) := \left\{\hat{u}_i(t) - u_i \leq \gamma_i(t)\right\}$.

Then, we have $\Pr\left(\mathcal{J}_i(t)\right)$
\begin{equation}\label{eq:prnf}
\begin{aligned}
   =& \Pr\left({\mathcal{J}_i(t)}|\mathcal{A}_i(t) \right) \Pr(\mathcal{A}_i(t)) + \Pr\left({\mathcal{J}_i(t)}|\overline{\mathcal{A}_i(t)} \right) \Pr(\overline{\mathcal{A}_i(t)})\\
   \leq&\Pr\left({\mathcal{J}_i(t)}|\mathcal{A}_i(t)\right) + \Pr\left(\overline{\mathcal{A}_i(t)}\right).
\end{aligned}
\end{equation}

Let $\mathbf{F}_{\alpha,\beta}^{Beta}(\cdot)$ denote the CDF of Beta distribution with parameters $\alpha$ and $\beta$, and $\mathbf{F}_{n,p}^{B}(\cdot)$ denote the CDF of Binomial distribution with parameters $n$ and $p$.

With above notations, we can bound $\Pr\left({\mathcal{J}_i(t)}|\mathcal{A}_i(t)\right)$ as follows:
\begin{equation}\label{eq:pra1}
\begin{aligned}
    \Pr\left({\mathcal{J}_i(t)}|\mathcal{A}_i(t)\right) =& \Pr\left(\theta_i(t)>u_i+2\gamma_i(t)|\mathcal{A}_i(t)\right)\\
    \stackrel{(\rm a)}{\leq} & \Pr\left(\theta_i(t)>\hat{u}_i(t) + \gamma_i(t)\right)\\
    = & \mathbb{E}\left[{\Pr\left(\theta_i(t)>\hat{u}_i(t)  + \gamma_i(t) | \mathcal{F}_{t-1} \right)}\right],
\end{aligned}
\end{equation}
where (a) is due to the fact that $u_i + 2\gamma_i(t) \geq \hat{u}_i(t) + \gamma_i(t)$ conditioned on $\mathcal{A}_i(t)$ happens.

Since given $\mathcal{F}_{t-1}$, $\hat{u}_i(t)$ and $\gamma_i(t)$ are determined, we have
\begin{equation}\label{eq:pra3}
\begin{aligned}
     &\Pr\left(\theta_i(t)>\hat{u}_i(t) + \gamma_i(t) | \mathcal{F}_{t-1} \right)\\ 
    =& 1-\mathbf{F}_{\alpha_i(t),\beta_i(t)}^{Beta}\left(\hat{u}_i(t) + \gamma_i(t)\right)  \\
    \stackrel{(\rm b)}{=}& \mathbf{F}_{\alpha_i(t)+\beta_i(t)-1,\hat{u}_i(t)+\gamma_i(t)}^{B}\left(\alpha_i(t)-1\right), \\
\end{aligned}
\end{equation}
where (b) is due to Fact 3 in \cite{Agrawal2017} for the relationship between Beta and Binomial distributions. 

Define $d(a,b)$ as the KL divergence between $a$ and $b$. Since $\alpha_i(t)-1 = \hat{u}_i(t)(\alpha_i(t)+\beta_i(t)-2)$, (\ref{eq:pra3}) can be further bounded by

\begin{equation}\label{eq:pra2}
    \begin{aligned}
    &\mathbf{F}_{\alpha_i(t)+\beta_i(t)-1,\hat{u}_i(t)+\gamma_i(t)}^{B}\left(\hat{u}_i(t)(\alpha_i(t)+\beta_i(t)-1)\right) \\
    \stackrel{(\rm a)}{\leq} & e^{-(\alpha_i(t)+\beta_i(t)-1)d(\hat{u}_i(t), \hat{u}_i(t)+\gamma_i(t))}\\
    \stackrel{(\rm b)}{\leq} & e^{-h_i(t)\frac{|\hat{u}_i(t)-\hat{u}_i(t)-\gamma_i(t)|^2}{2}}\\
    =& e^{-h_i(t)\frac{\gamma^2_i(t)}{2}}\\
    =& \frac{1}{T},
    \end{aligned}
\end{equation}
where (a) is due to Fact 1 in \cite{Agrawal2017} by the Chernoff-Hoeffding bound and (b) is due to the fact that $d(a,b)\geq \frac{|a-b|^2}{2}$.
Substituting (\ref{eq:pra2}) and (\ref{eq:pra3}) into (\ref{eq:pra1}), we have
\begin{equation}\label{eq:pra4}
\begin{aligned}
    \Pr\left({\mathcal{J}_i(t)}|\mathcal{A}_i(t)\right)\leq \frac{1}{T}.
\end{aligned}
\end{equation}

On the other hand, $\Pr\left(\overline{\mathcal{A}_i(t)}\right)$ can be written as
\begin{equation*}\label{eq:prna1}
    \Pr\left(\overline{\mathcal{A}_i(t)}\right) = \mathbb{E}\left[\Pr\left(\overline{\mathcal{A}_i(t)} | \mathcal{F}_{t-1}\right)\right].
\end{equation*}
Given $\mathcal{F}_{t-1}$,  $\hat{u}_i(t)$ and $\gamma_i(t)$ are determined. Then also by Chernoff-Hoeffding inequality (Fact 2 in \cite{Agrawal2017}), we have
\begin{equation*}\label{eq:prna}
    \begin{aligned}
        \Pr\left(\overline{\mathcal{A}_i(t)}| \mathcal{F}_{t-1}\right) =& \Pr(\hat{u}_i(t) - u_i > \gamma_i(t))\\
        \leq& e^{-2 (\gamma_i(t))^2h_i(t)}=\frac{1}{T^4}.
    \end{aligned}
\end{equation*}
Therefore,  we have
\begin{equation}\label{eq:prna3}
    \Pr\left(\overline{\mathcal{A}_i(t)}\right) \leq \frac{1}{T^4}
\end{equation}

Substituting (\ref{eq:prna3}), (\ref{eq:pra4}) into (\ref{eq:prnf}) concludes the proof.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma \ref{lm:kt}}
\begin{proof}
Define event $\mathcal{G}_i(t)$ as
\begin{equation*}
    \mathcal{G}_i(t) := \{u_i-\hat{u}_i(t) \leq \varepsilon_i(t)\}.
\end{equation*}
We can decompose $\Pr\left({\mathcal{K}_i(t)}\right)$ as follows
\begin{equation}\label{eq:prnk}
\begin{aligned}
    &\Pr\left({\mathcal{K}_i(t)}|\mathcal{G}_i(t) \right) \Pr(\mathcal{G}_i(t)) + \Pr\left({\mathcal{K}_i(t)}|\overline{\mathcal{G}_i(t)} \right) \Pr(\overline{\mathcal{G}_i(t)})\\
   \leq&\Pr\left({\mathcal{K}_i(t)}|\mathcal{G}_i(t)\right) + \Pr\left(\overline{\mathcal{G}_i(t)}\right).
\end{aligned}
\end{equation}
For each arm $i$, since $u_i-2\varepsilon_i(t)\leq \hat{u}_i(t)-{\varepsilon_i(t)}$ when $\mathcal{G}_i(t)$ happens, we have $\Pr\left(\theta_i(t)<u_i-2\varepsilon_i(t)|\mathcal{G}_i(t)\right)$ bounded by
\begin{equation}\label{eq:pr1}
\begin{aligned}
     & \Pr\left(\theta_i(t)<\hat{u}_i-\varepsilon_i(t)\right)=  \mathbb{E}\left[\Pr\left(\theta_i(t)<\hat{u}_i-\varepsilon_i(t) | \mathcal{F}_{t-1}  \right) \right]
\end{aligned}
\end{equation}
Given $\mathcal{F}_{t-1}$, $\hat{u}_i(t)$ and $\varepsilon_i(t)$ are determined. Then, we can write $\Pr\left(\theta_i(t)<\hat{u}_i(t)-\varepsilon_i(t) | \mathcal{F}_{t-1}\right)$ as
\begin{equation}\label{eq:pr11}
\begin{aligned}
     &\mathbf{F}_{\alpha_i(t), \beta_i(t)}^{Beta}(\hat{u}_i(t)-{\varepsilon_i(t)})\\
     = & 1 -  \mathbf{F}_{\alpha_i(t) + \beta_i(t)-1, \hat{u}_i(t)-{\varepsilon_i(t)}}^{B}(\alpha_i(t)-1) \\
      \stackrel{(\rm b)} {=} & 1 -  \mathbf{F}_{h_i(t) + 1, \hat{u}_i(t)-{\varepsilon_i(t)}}^{B}(\hat{u}_i(t) h_i(t)),
\end{aligned}
\end{equation}
where  (b) is due to $h_i(t) = \alpha_i(t) + \beta_i(t)-2$ and $\alpha_i(t)-1 = \hat{u}_i(t)h_i(t)$.

%Next, we prove $\mathbf{F}_{h_i(t) + 1, \hat{u}_i-{\varepsilon_i(t)}}^{B}(\hat{u}_i h_i(t))$ is lower bounded. 
Let $Y_{j}$ be an outcome of the $j$-th Bernoulli trial with mean value $\hat{u}_i(t)-{\varepsilon_i(t)}$. $S_i := \sum\limits_{j=1}^{h_i(t)+1} Y_j$ is a random variable generated from Binomial distribution with parameters $h_i(t) + 1$~(number of trials) and $\hat{u}_i(t)-{\varepsilon_i(t)}$~(mean value). Then, we have
\begin{equation}\label{eq:Fb1m}
\begin{aligned}
    F_{h_i(t) + 1, \hat{u}_i(t)-{\varepsilon_i(t)}}^{B}(\hat{u}_i(t) h_i(t)) =& \Pr\left(S_i \leq \hat{u}_i(t) h_i(t)\right) \\
    = & 1 - \Pr\left(S_i > \hat{u}_i(t) h_i(t)\right).
\end{aligned}
\end{equation}
Substituting (\ref{eq:Fb1m}) into (\ref{eq:pr11}), we have
\begin{equation}\label{eq:fb2m}
    \mathbf{F}_{\alpha_i(t), \beta_i(t)}^{Beta}(\hat{u}_i(t)-{\varepsilon_i(t)})=\Pr\left(S_i > \hat{u}_i h_i(t)\right).
\end{equation}
We can rewrite $\Pr\left(S_i > \hat{u}_i h_i(t)\right)$ as
\begin{equation*}\label{eq:lema22}
\begin{aligned}
\Pr\left(S_i > n \mathbb{E}[Y_j]+\delta_i\right),
\end{aligned}
\end{equation*}
where $n=h_i(t)+1$, $\mathbb{E}[Y_j]=\hat{u}_i(t)-{\varepsilon_i(t)}$, and $\delta_i = \hat{u}_i(t) h_i(t)-(\hat{u}_i(t)-{\varepsilon_i(t)})(h_i(t)+1)$.

Therefore, according to the Chernoff–Hoeffding bound (Fact 2 in \cite{Agrawal2017}), we have 
\begin{equation*}
\begin{aligned}
    &\Pr\left(S_i > \hat{u}_i(t) h_i(t)\right)\\
    \leq& e^{-2(\delta_i)^2/n^2}\\
    =&e^{-2 \left(\hat{u}_i(t) h_i(t) - (\hat{u}_i(t)-{\varepsilon_i(t)})(h_i(t)+1)\right)^2/(h_i(t)+1)}\\
    =& e^{-2(\hat{u}^2_i(t) -  2 \hat{u}_i(t) \varepsilon_i(t)  (h_i(t)+1) + {\varepsilon_i(t)^2}(h_i(t)+1)^2)/(h_i(t)+1)} \\
    \leq & e^{-2( -  2 \hat{u}_i(t) \varepsilon_i(t) + {\varepsilon_i(t)^2}(h_i(t)+1))}\\
    = & e^{4 \hat{u}_i(t) \varepsilon_i(t) -2{\varepsilon_i(t)^2}(h_i(t)+1)}\\
    \leq & e^{4 \varepsilon_i(t) -2{\varepsilon_i(t)^2}h_i(t)}.
\end{aligned}
\end{equation*}
When  $h_i(t) \geq 4$, we have $h_i(t) \geq \frac{8}{\ln t}$, which means $4 \varepsilon_i(t) \leq \varepsilon^2_i(t)h_i(t)$. Then,
\begin{equation}\label{eq:g1}
\begin{aligned}
    \Pr\left(S_i > \hat{u}_i(t) h_i(t)\right) \leq e^{4 \varepsilon_i(t) -2{\varepsilon_i(t)^2}h_i(t)} \leq e^{-{\varepsilon_i^2(t)}h_i(t)}  = \frac{1}{t^2}.
\end{aligned}    
\end{equation}
Substituting (\ref{eq:g1}) into (\ref{eq:fb2m}), we have
\begin{equation*}
    \Pr\left(\theta_i(t)<\hat{u}_i(t)-\varepsilon_i(t) | \mathcal{F}_{t-1}  \right) \leq \frac{1}{t^2}.
\end{equation*}
Therefore,
\begin{equation*}\label{eq:t22}
    \Pr\left(\theta_i(t)<\hat{u}_i(t)-\varepsilon_i(t)\right) \leq \mathbb{E}\left[\Pr\left(\theta_i(t)<\hat{u}_i(t)-\varepsilon_i(t) | \mathcal{F}_{t-1}  \right) \right] = \frac{1}{t^2}.
\end{equation*}
On the other hand, $\Pr \left( \overline{\mathcal{G}_i(t)} \right) = \mathbb{E}\left[\Pr \left( \overline{\mathcal{G}_i(t)} | \mathcal{F}_{t-1} \right) \right]$. Given $\mathcal{F}_{t-1}$, $\hat{u}_i(t)$ and $\epsilon_i(t)$ is determined, and $\Pr \left( \overline{\mathcal{G}_i(t)} | \mathcal{F}_{t-1} \right)$ can be bounded by the Chernoff–Hoeffding bound (Fact 2 in \cite{Agrawal2017}) :
\begin{equation*}
\begin{aligned}
    \Pr \left( \overline{\mathcal{G}_i(t)}| \mathcal{F}_{t-1} = F_{t-1} \right)=& \Pr \left(\hat{u}_i(t) \leq u_i - {\varepsilon_i(t)} | \mathcal{F}_{t-1} = F_{t-1} \right)\\
    \leq & e^{-2 ({\varepsilon_i(t)})^2 h_i(t)}\\
    =& \frac{1}{t^4}.
\end{aligned}
\end{equation*}
Therefore, $\Pr \left( \overline{\mathcal{G}_i(t)} \right)$ can be bounded by $\frac{1}{t^4}$
\end{proof}


\subsubsection{Proof of Lemma \ref{lm:gs}}
\begin{proof}
Let event $\mathcal{C}_i(t)$ be defined as
\begin{equation*}
    \mathcal{C}_i(t) := \left\{\hat{u}_i(t) - u_i \leq \gamma_i(t)\right\}.
\end{equation*}
Then, $\Pr\left({\mathcal{J}_i(t)}\right)$ can be written as
\begin{equation}\label{eq:prnh}
\begin{aligned}
   &\Pr\left({\mathcal{J}_i(t)}|\mathcal{C}_i(t) \right) \Pr(\mathcal{C}_i(t)) + \Pr\left({\mathcal{J}_i(t)}|\overline{\mathcal{C}_i(t)} \right) \Pr(\overline{\mathcal{C}_i(t)})\\
   \leq&\Pr\left({\mathcal{J}_i(t)}|\mathcal{C}_i(t)\right) + \Pr\left(\overline{\mathcal{C}_i(t)}\right).
\end{aligned}
\end{equation}
Since  $u_i + 2\gamma_i(t) \geq \hat{u}_i(t) + \gamma_i(t)$ when $\mathcal{C}_i(t)$ happens, $\Pr\left({\mathcal{J}_i(t)}|\mathcal{C}_i(t)\right)$ can be bounded by
\begin{equation*}
\begin{aligned}
    &\Pr\left(\theta_i(t) > \hat{u}_i(t) + \gamma_i(t)\right)\\
    =& \mathbb{E}\left[\Pr\left(\theta_i(t) > \hat{u}_i(t) + \gamma_i(t) | \mathcal{F}_{t-1}\right)\right].
\end{aligned}
\end{equation*}
Given $\mathcal{F}_{t-1}$, $\hat{u}_i(t)$ and $\gamma_i(t)$ are determined. Then according to Fact 4 in \cite{Agrawal2017} for the concentration of Gaussian distributions, we have
\begin{equation*}
\begin{aligned}
    \Pr\left(\theta_i(t) > \hat{u}_i(t) + \gamma_i(t) | \mathcal{F}_{t-1}\right)
    \leq& \frac{1}{2} e^{-(\gamma_i(t)\cdot (h_i(t)+1))^2/2}\\
    \leq& \frac{1}{2} e^{-(\gamma_i(t)\cdot (h_i(t)))^2/2}\\
    =& \frac{1}{2}  \frac{1}{T^{h_i(t)}}\\
    \leq& \frac{1}{T}.
\end{aligned}
\end{equation*}
where the last inequality is due to the condition $h_i(t) > 0$.
Therefore, $\Pr\left({\mathcal{J}_i(t)}|\mathcal{C}_i(t)\right)$ can be bounded by $\frac{1}{T}$.

On the other hand, by the Chernoff–Hoeffding bound, we have
\begin{equation*}
    \Pr\left(\overline{\mathcal{C}_i(t)}\right) \leq \frac{1}{T^4},
\end{equation*}
Therefore, $\Pr\left({\mathcal{J}_i(t)}\right)$ can be bounded by $\frac{1}{T}+\frac{1}{T^4}$.

$\Pr\left(\overline{\mathcal{H}_i(t)}\right)$ can be bounded in the same way.
\end{proof}







==> Thompson Sampling for Combinatorial Semi-bandits with Sleeping Arms and Long-Term Fairness Constraints/0-Abstract.tex <==
\begin{abstract}
We study the combinatorial sleeping multi-armed semi-bandit problem with long-term fairness constraints~(CSMAB-F).
To address the problem, we adopt Thompson Sampling~(TS) to maximize the total rewards and use virtual queue techniques to handle the fairness constraints, and design an algorithm called \emph{TS with beta priors and Bernoulli likelihoods for CSMAB-F~(TSCSF-B)}.
Further, we prove TSCSF-B can satisfy the fairness constraints, and the time-averaged regret is upper bounded by $\frac{N}{2\eta} + O\left(\frac{\sqrt{mNT\ln T}}{T}\right)$, where $N$ is the total number of arms, $m$ is the maximum number of arms that can be pulled simultaneously in each round~(the cardinality constraint) and $\eta$ is the parameter trading off fairness for rewards. By relaxing the fairness constraints (i.e., let $\eta \rightarrow \infty$), the bound boils down to the first problem-independent bound of TS algorithms for combinatorial sleeping multi-armed semi-bandit problems.
Finally, we perform numerical experiments and use a high-rating movie recommendation application to show the effectiveness and efficiency of the proposed algorithm.
\end{abstract}

==> Thompson Sampling for Combinatorial Semi-bandits with Sleeping Arms and Long-Term Fairness Constraints/1-Introduction.tex <==
\section{Introduction}
% the problem
% Bingshan starts to revise {This part is the stochastic bandit feedback

%Multi-armed bandits (MAB) are one of the most often used approaches to model sequential learning and decision-making problems, including the application of resource allocation in computer and communication systems. In the most basic setting, i.e., \emph{stochastic} MAB problems, arms (i.e., resource requests) are associated with random rewards that are i.i.d. drawn from fixed but unknown distributions. Here reward is a very generic term and can be defined based on different scenarios (e.g., success probability, return on investment, and so on~\cite{bubeck2012regret}). The goal of a learning agent is to pull arms sequentially to accumulate rewards as many as possible over $T$ rounds. However, in each round, the learning agent can only observe the random reward of the pulled arm. Therefore, this partial information feedback mechanism forces the learning agent to face the exploration and exploitation dilemma, i.e., in each round, the agent can either do exploration (acquiring information to estimate the mean reward of each arm) or exploitation (achieving rewards as many as possible).

%}

% Bingshan starts to revise {This part will be the regret and problem dependent and problem independent regret bound)

%}

% Bingshan starts to revise {This part talks about the classic no-regret algorithm)

%There are two well-known algorithms to address the stochastic MAB problems. One is the \emph{Upper Confidence Bound (UCB)} algorithm~\cite{auer2002finite}, where each arm is represented by a confidence interval centering on the sample mean (empirical mean). In each round, the  agent pulls the arm with the highest upper confidence bound (the empirical mean plus the confidence interval). 
%Note that UCB algorithm is deterministic as there is no randomization within the algorithm itself. Instead, the adaptive confidence interval is used to achieve the balance between exploration and exploitation.
%The other one is the \emph{Thompson Sampling (TS)} algorithm due to William Thompson in 1930’s. TS assumes a simple prior distribution over the underlying parameters of the reward distributions of all the arms. In each round, the agent draws a random sample from the distribution for each arm and then pulls the arm with the highest posterior sample value.

%Practically, TS usually outperforms UCB-based algorithms significantly~\cite{chapelle2011empirical}. Theoretically, TS is comparable to UCB~\cite{hu2019problem,Agrawal2017} while 

%The quality of the learning algorithms is measured by \emph{regret}. The regret is defined as the cumulative performance gap between always pulling the arm with the highest mean reward and the arms  recommended by the learning algorithms. If a regret bound depends on a specific problem instance, we call it a \emph{problem-dependent} regret bound while if a regret bound does not depend on any problem instances, we call it a \emph{problem-independent} regret bound. For the simplicity of presenting the difference between problem-dependent regret bounds and problem-independent regret bounds, we consider a stochastic $N$-armed bandit problem with one arm having mean reward $u$ and all the remaining arms having the mean reward $u-\Delta, \Delta > 0$. In this setting, the problem-dependent regret bound takes the form $O \left(\frac{   N \log T}{\Delta}   \right)$~\cite{auer2002finite} or $O \left( \frac{N \Delta \log T}{d(u-\Delta, u)}  \right)$~\cite{Agrawal2017}  while the problem-independent regret bound takes the form $\widetilde{O} \left( \sqrt{NT}  \right)$~\cite{auer2010ucb,Agrawal2017}~\footnote{We use $d(p,q):= p \log \frac{p}{q} + (1-p) \log \frac{1-p}{1-q}$ to denote the KL divergence between two Bernoulli distributions with means $p$ and $q$, and use $\widetilde{O}(\cdot)$ to hide logarithmic factors.}.


%Due to MAB’s powerful capability to capture real-world problems, many research efforts have been spent in the last half-century on different MAB variants. One of the most important variants is the combinatorial MAB (CMAB) with semi-bandit feedback as in some practical applications, the learning agent needs to pull more than one arm simultaneously. In this setting, multiple arms subject to certain constraints can be pulled simultaneously in each round and the semi-bandit feedback ensures that the reward of each individual arm can be observed~\cite{gai2012combinatorial,chen2013combinatorial,kveton2015tight,wang2018thompson,Kveton2014matroid,komiyama2015optimal}. However, all these works have assumed that the learning agent can pull arms from a fixed arm set, i.e., the set of available arms does not vary in each round. The works \cite{kleinberg2010regret,Chatterjee2017AnalysisOT,hu2019int,NIPS2016_6450,NIPS2014_5381} have considered a more advanced setting that the set of available arms can vary in each round. We call this setting the \emph{CMAB with sleeping arms}~(CSMAB). In this setting, some arms may be sleeping (i.e., unavailable) in some certain rounds and the \emph{availability set}, the set that collects all the available arms in each round, can be decided either in a stochastic way or in an adversarial way.


%following unknown distributions and parameters, but the arm availability is revealed at the beginning of each round, so only available arms can be pulled in each round, etc. 

In this paper, we focus on a recent variant of \emph{multi-armed bandit~(MAB)} problems, which is the combinatorial sleeping MAB with long-term fairness constraints (CSMAB-F)~\cite{li2019combinatorial}. In CSMAB-F, a learning agent needs to simultaneously pull a subset of available arms subject to some constraints~(usually the cardinality constraint) and only observes the reward of each pulled arm~(semi-bandit setting) in each round. Both the availability and the reward of each arm are stochastically generated, and the long-term fairness among arms is further considered, i.e., each arm should be pulled at least a number of times in a long horizon of time. The objective is to accumulate as many rewards as possible in the finite time horizon. 
The CSMAB-F problem has a wide range of real-world applications. For example, in task assignment problems, we want each worker to be assigned for a certain number of tasks~(i.e., fairness constraints), while some of the workers may be unavailable in some time slots~(i.e., sleeping arms). In movie recommendation systems considering movie diversity, different movie genres should be recommended for a certain number of times~(i.e., fairness constraints), while we do not recommend users with genres they dislike~(i.e., sleeping arms).

\emph{Upper Confidence Bound (UCB)} and \emph{Thompson Sampling (TS)} are two well-known families of algorithms to address the stochastic MAB problems. Theoretically, TS is comparable to UCB~\cite{hu2019problem,Agrawal2017}, but practically, TS usually outperforms UCB-based algorithms significantly~\cite{chapelle2011empirical}. However, while the theoretical performance of UCB-based algorithms has been extensively studied for various MAB problems~\cite{bubeck2012regret}, there are only a few theoretical results for TS-based algorithms~\cite{Agrawal2017,Chatterjee2017AnalysisOT,wang2018thompson}.

In ~\cite{li2019combinatorial}, a UCB-based algorithm called \emph{Learning with Fairness Guarantee~(LFG)} was devised and a problem-independent regret bound \footnote{If a regret bound depends on a specific problem instance, we call it a \emph{problem-dependent} regret bound while if a regret bound does not depend on any problem instances, we call it a \emph{problem-independent} regret bound.} $\frac{N}{2\eta} + \frac{2\sqrt{6mNT\ln T}+ 5.11w_{\max}N }{T}$ was derived for the CSMAB-F problem, where $N$ is the number of arms, $m$ is the maximal number of arms that can be pulled simultaneously in each round, $w_{\max}$ is the maximum arm weight,  and  $\eta$ is a parameter that balances the the fairness and the reward. However, as TS-based algorithms are usually comparable to UCB theoretically but practically perform better than UCB, we are motivated to devise TS-based algorithms and derive regret bounds of such algorithms for the CSMAB-F problem.
The contributions of this paper can be summarized as follows. 
\begin{itemize}[leftmargin=*]
    \item We devise the first TS-based algorithm for CSMAB-F problems with a provable upper regret bound. To be fully comparable with LFG, we incorporate the virtual queue techniques defined in~\cite{li2019combinatorial} but make a modification on the queue evolution process to reduce the accumulated rounding errors.
    \item Our regret bound~$\frac{N}{2\eta} + \frac{4\sqrt{mNT\ln T}+ 2.51w_{\max}N }{T}$ is in the same polynomial order as the one achieved by LFG, but with lower coefficients. This fact shows again that TS-based algorithms can achieve comparable theoretical guarantee as UCB-based algorithms but with a tighter bound.
    
    %This shows again that TS-based approaches are intrinsically more effective than UCB-based ones. Although TSCSF-B and TSCSF-G have a slightly higher coefficient for time-independent regret components as TS-based algorithms for other MAB problems, when the number ($N$) of arms is much less than $T$, which is often the case of interest in practice, such components are totally negligible.
    
    \item We verify and validate the practical performance of our proposed algorithms by numerical experiments and real-world applications. Compared with LFG, it is shown that TSCSF-B does perform better than LFG in practice.
\end{itemize}
%even though the bounds are in the same order of magnitude as LFG, similar to UCB and TS-based algorithms for ordinary MAB problems, both TSCSF-B and TSCSF-G have a lower coefficient for time-related regret components. 
  It is noteworthy that our algorithmic framework and proof techniques are extensible to other MAB problems with other fairness definitions. Furthermore, if we do not consider the fairness constraints, our bound boils down to the first problem-independent upper regret bounds of TS algorithms for CSMAB problems and matches the lower regret bound~\cite{bubeck2012regret}.


%the efficiency in both achieved regrets and convergence behaviors of TSCSF-B and TSCSF-G. 




% the structure

The remainder of this paper is organized as follows. In Section~\ref{sec:related}, we summarize the most related works about CSMAB-F. The problem formulation of CSMAB-F is presented in Section~\ref{sec:problem}, following what in \cite{li2019combinatorial} for comparison purposes. The proposed TS-based algorithm is presented in Section~\ref{sec:algorithms}, with main results, i.e., the fairness guarantee, performance bounds and proof sketches, presented in Section~\ref{sec:results}. 
%Proof sketches are given in Section~\ref{sec:proofs} with details in the Appendix. 
Performance evaluations are presented in Section~\ref{sec:evaluation}, followed by concluding remarks and future work in Section~\ref{sec:conclusion}. Detailed proofs can be found in Appendix \ref{sec:appendix}.

==> Thompson Sampling for Combinatorial Semi-bandits with Sleeping Arms and Long-Term Fairness Constraints/2-RelatedWorks.tex <==
\section{Related Works}\label{sec:related}

%We start with the classic stochastic MAB problem, which is the most widely studied version of MAB problems.
%There are two families of algorithms that can successfully address the exploration and exploitation dilemma: the UCB-based algorithms and the TS-based algorithms. UCB-based algorithms are deterministic conditioned on the history information, which constructs a confidence radius to estimate the mean rewards of arms in each round. The advantage of UCB-based algorithms is that they have theoretical guarantees in many complicated bandit settings and do not require the stochastic reward of each arm to be independent. However, in some scenarios where the reward of each arm is drawn from an independent distribution, TS-based algorithms are shown to have a better performance than UCB-based algorithms~\cite{chapelle2011empirical}. 


%One of the widely used and easy-to-implement algorithms is the Upper Confidence Bound (UCB) algorithm proposed in \cite{auer2002finite}. It achieves problem-dependent regret bounds in the form either $O \left(\frac{   K \log T}{\Delta}   \right)$~\cite{auer2002finite} or $O \left( \frac{K \Delta \log T}{d(\mu-\Delta, \mu)}  \right)$ and problem-independent regret bound 



%. Since the coefficient of the logarithmic term in the UCB regret is larger than the theoretical lower bound in \cite{lai1985asymptotically}, many variants of UCB algorithm are proposed to improve the bound, such as Bayes-UCB \cite{kaufmann2012bayesian}, KL-UCB \cite{garivier2011kl}. On the other hand, Thompson sampling is also an alternative way to solve stochastic MAB problems and is shown to have a better performance than UCB algorithms in practice~\cite{chapelle2011empirical}. Recently, the logarithmic bound on expected regret of TS is proven in \cite{Agrawal2017} and \cite{kaufmann2012thompson}, which matches the theoretical lower bound in \cite{lai1985asymptotically}.


% Put it here tentatively




% Bingshan starts to revise

Many variants of the stochastic MAB problems have been proposed and the corresponding regret bounds have been derived. The ones that are most related to our work are \emph{Combinatorial MAB (CMAB)} and its variants, which was first proposed and analyzed in \cite{gai2012combinatorial}. In CMAB, an agent needs to pull a combination of arms simultaneously from a fixed arm set. Considering a semi-bandit feedback setting, i.e., the individual reward of each arm in the played combinatorial action can be observed, the authors of \cite{chen2013combinatorial} derived a sublinear problem-dependent upper regret bound based on a UCB algorithm and this bound was further improved in \cite{kveton2015tight}. In \cite{combes2015combinatorial}, a problem-dependent lower regret bound was derived by constructing some problem instances. Very recently, the authors of \cite{wang2018thompson} derived a problem-dependent regret bound of TS-based algorithms for CMAB problems. %and matroid bandit problems~\cite{Kveton2014matroid}. 

All the aforementioned works make an assumption that the arm set from which the learning agent can pull arms is fixed over all $T$ rounds, i.e., all the arms are always available and ready to be pulled. However, in practice, some of the arms may not be available in some rounds, for example, some items for online sales are out of stock temporarily. Therefore, a bunch of literature studied the setting of \emph{MAB with sleeping arms (SMAB)} ~\cite{kleinberg2010regret,Chatterjee2017AnalysisOT,hu2019int,NIPS2016_6450,NIPS2014_5381}.  In the SMAB setting, the set of available arms for each round, i.e., the availability set, can vary. For the simplest version of SMAB (only one arm is pulled in each round), the problem-dependent regret bounds of UCB-based algorithms and TS-based algorithms have been analyzed in \cite{kleinberg2010regret} and \cite{Chatterjee2017AnalysisOT}, respectively.

Regarding the combinatorial SMAB setting~(CSMAB), some negative results are shown in \cite{NIPS2016_6450}, i.e., efficient no-regret learning algorithms sometimes are computationally hard. However, for some settings such as stochastic availability and stochastic reward,  it is shown that it is still possible to devise efficient learning algorithms with good theoretical guarantees \cite{hu2019int,li2019combinatorial}. More importantly, in the work of  \cite{li2019combinatorial}, they considered a new variant called the \emph{combinatorial sleeping MAB with long-term fairness constraints (CSMAB-F)}. In this setting, fairness among arms is further considered, i.e., each arm needs to be pulled for a number of times. The authors designed a UCB-based algorithm called \emph{Learning with Fairness Guarantee~(LFG)} and provided a problem-independent time-averaged upper regret bound.
%$\frac{N}{2 \eta} + O\left(\frac{\sqrt{mNT\ln T}}{T}\right)$. 
%Note that when $\eta = \infty$, it means fairness is neglected and the algorithm only wants to achieve reward maximization. 

Due to the attractive practical performance and lack of theoretical guarantees for TS-based algorithms in CSMAB-F, it is desirable to devise a TS-based algorithm and derive regret bounds for such algorithms. We are interested to derive the problem-independent regret bound as it holds for all problem instances. In this work, we give the first provable regret bound that is in the same polynomial order as the one in \cite{li2019combinatorial} but with lower coefficients.  To the best of our knowledge, the derived upper bound is also the first problem-independent regret bound of TS-based algorithms for CSMAB problems which matches the lower regret bounds~\cite{kveton2015tight} when relaxing the long-term fairness constraints.


%In SMAB, a set of arms will be unavailable to pull at the beginning of each round.  It is shown in \cite{NIPS2016_6450} that several online problems with sleeping settings that admit efficient no-regret algorithms become computationally hard. Further, The authors of \cite{kleinberg2010regret} provide a lower regret bound for any algorithm, and a upper bound for a UCB-based algorithm in SMAB.

%Recently, a problem-dependent regret bound of TS in SMAB is analyzed in \cite{Chatterjee2017AnalysisOT}, which matches the lower bound. 




%The settings combined CMAB with SMAB are known as combinatorial sleeping MAB~(CSMAB). A problem-dependent bound is given in \cite{hu2019int} when both the availability and rewards of arms are stochastic. On the other hand, the authors of \cite{NIPS2014_5381} analyze the effect of arms with stochastic availability and adversarial rewards.
%However, there is no regret bound for TS algorithm in CSMAB. 


% Bingshan starts



%The fairness constraints in MAB problems are studied in many works with different fairness definitions. In \cite{joseph2016fairness}, the fairness is that two arms should be pulled with the same probability until they can be distinguished with high confidence. On the other hand, the fairness in \cite{talebi2018learning} is studied in a resource allocation problem, where all tasks of a job should be served at the same rate by a fixed number of servers. 


%In our work, we consider the fairness constraints as the minimum number of times that an arm should be pulled. Therefore, the above studies have less relevance to our work.


% Bingshan starts
%More recently, the work of \cite{li2019combinatorial} 



%TS in CSMAB-F and give the first time-averaged regret bounds for TS algorithms of $\frac{N}{2 \eta} + O\left(\frac{\sqrt{mNT\ln T}}{T}\right)$, where the coefficient of our leading term (the term depends on $T$) is smaller than the bound of LFG. It is also noteworthy that by neglecting fairness constraints~(let $\eta = \infty$), our bounds are the first problem-independent bounds for TS algorithms in CSMAB, which matches the problem-independent bounds in \cite{Agrawal2017}.

==> Thompson Sampling for Combinatorial Semi-bandits with Sleeping Arms and Long-Term Fairness Constraints/3-Problem.tex <==
\section{Problem Formulation}\label{sec:problem}
In this section, we present the problem formulation of the stochastic combinatorial sleeping multi-armed bandit problem with fairness constraints~(CSMAB-F), following ~\cite{li2019combinatorial} closely for comparison purposes. To state the problem clearly, we first introduce the CSMAB problem and then incorporate the fairness constraints.


Let set $\mathcal{N} := \{1,2,\ldots,N\}$ be an arm set and $\Theta := 2^{\mathcal{N}}$ be the power set of $\mathcal{N}$. At the beginning of each round $t = 0, 1, \ldots, T-1$, a set of arms $Z(t) \in \Theta$ are revealed to a learning agent according to a fixed but unknown distribution $P_{Z}$ over $\Theta$, i.e., $P_{Z}: \Theta \rightarrow [0,1]$. We call set $Z(t)$ the \emph{availability set in round $t$}. Meanwhile, each arm $i \in \mathcal{N}$ is associated with a random reward $X_i(t) \in \{0,1\}$ drawn from a fixed Bernoulli distribution $D_i$ with an unknown mean $u_i := \mathbb{E}_{X_i(t) \sim D_i} \left[ X_i \right]$~\footnote{Note that we only consider Bernoulli distribution in this paper for brevity, but it is feasible to extend our algorithm and analysis with little modifications to other general distributions~(see \cite{agrawal2012analysis,Agrawal2017}).}, and a fixed known non-negative weight $w_i$ for that arm. Note that for all the arms in $\mathcal{N}$, their rewards are drawn independently in each round $t$.
%a unit cube $[0, 1]^{\Theta}$, i.e., $P_Z(S) := \Pr(Z(t) = S), \forall S \in \Theta$. 
Then the learning agent pulls a subset of arms $A(t)$ from the availability set with the cardinality no more than $m$, i.e., $A(t) \subseteq Z(t), |A(t)|\leq m$, and receives a weighted random reward $R(t) := \sum_{i \in A(t)} w_i X_i(t)$. 

In this work,  we consider the semi-bandit feedback setting, which is consistent with \cite{li2019combinatorial}, i.e., the learning agent can observe the individual random reward of all the arms in $A(t)$. Note that since the availability set $Z(t)$ is drawn from a fixed distribution $P_{Z}$ and the random rewards of the arms are also drawn from fixed distributions, we are in a bandit setting called the \emph{stochastic availability} and the \emph{stochastic reward}. 

%receives feedback $Q(t) = \{(i,X_i(t))|i\in A(t)\}$.


The objective of the learning agent is to pull the arms sequentially to maximize the expected time-averaged rewards over $T$ rounds, i.e., $\max \mathbb{E}\left[\frac{1}{T}\sum_{t=0}^{T-1} R(t)\right] $. 

Furthermore, we consider the long-term fairness constraints proposed in \cite{li2019combinatorial}, where 
each arm $i \in \mathcal{N}$ is expected to be pulled at least $k_i \cdot T$ times when the time horizon is long enough, i.e.,
%with a predefined value $k_i \in [0, p_i]$, where $p_i:=\sum\limits_{S\in \Theta : i \in S} P_Z(S)$ is the availability of arm $i$. 
\begin{equation}\label{eq:fraction}
    \liminf _{T \rightarrow \infty} \frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E}\left[\mathbf{1}[i \in A(t)]\right] \geq k_{i}, \forall i \in \mathcal{N}.
\end{equation}
We say a vector $\mathbf{k} := \begin{bmatrix}
k_1 & k_2 & \cdots & k_N
\end{bmatrix}^T$ is feasible if there exists a policy such that (\ref{eq:fraction}) is satisfied.

% Since the agent cannot pull more than $m$ arms simultaneously, the choice of each $k_i$ should comply with the constraint that $\sum\limits_{i \in \mathcal{N}} k_i \leq m$. 
% Otherwise, there may not be  feasible solution to satisfy the fairness constraints. Let vector $\mathbf{k} := \begin{bmatrix}
% k_1 & k_2 & \cdots & k_n
% \end{bmatrix}^T$. We say $\mathbf{k}$ is feasible if all of its elements satisfy the aforementioned requirements.

%where $k_{i}\in (0,1)$ is the minimum fraction of rounds that arm $i$ should be pulled. Define $\mathbf{k}:=[k_1 \quad k_2 \quad \cdots  \quad k_N]$ as a minimum fraction vector, which is \emph{feasible} only if there exists a policy that makes a sequence of decisions $A(t)$ for $t\geq0$ such that (\ref{eq:fraction}) is satisfied. All feasible vectors $\mathbf{k} \in (0,1)^N$ forms a set called the \emph{maximal feasibility region} $\mathbb{C}$. If there is a policy such that (\ref{eq:fraction}) is satisfied for any $\mathbf{k}$ strictly inside $\mathbb{C}$, we call the policy is \emph{feasibility-optimal}.

%Intuitively, the fairness constraints ensure that each arm $i$ will be pulled at least $k_i \cdot T$ times on expectation. 
% To introduce the optimal solution to the CSMAB-F problem, we consider such a policy which in each round
% chooses solution $A$ with probability $q_S(A) := \Pr(A(t) = A), A \subseteq S : |A| \leq m$ when observing a set of available arms $S \in \Theta$. Note that $\sum\limits_{A \subseteq S : |A|\leq m} q_{S}(A)=1, \forall S \in \Theta$. We call the policy $S$-only policy since the decision depends on the availability set $S \in \Theta$. Then, the fairness constraints defined in (\ref{eq:fraction}) can be converted to
% \begin{equation}
%     \sum\limits_{S \in \Theta} P_{Z}(S) \sum\limits_{A \subseteq S, |A|\leq m : i \in A} q_{S}(A) \geq k_{i}, \forall i \in \mathcal{N},
% \end{equation}
% where the left hand side is the expectation on the number of times that arm $i$ can be pulled in each round.
% The following Lemma from \cite{li2019combinatorial} states that there exists an optimal $S$-only policy:

If we knew the availability set distribution $P_{Z}$ and the mean reward $u_i$ for each arm $i$ in advance, and $\mathbf{k}$ was feasible, then there would be a randomized algorithm which is the optimal solution for CSMAB-F problems. The algorithm chooses arms $A(t)\subseteq S$ with probability $q_S(A)$ when observing available arms $S \in \Theta$.  Let $\mathbf{q}:=\{q_S(A), \forall S \in \Theta, \forall A \subseteq S : |A| \leq m \}$. We can determine $\mathbf{q}$ by solving the following problem:
\begin{equation}\label{eq:question}
\resizebox{.9\hsize}{!}{$
    \begin{array}{ll}{
    \underset{\mathbf{q}}{\operatorname{maximize}}} & {\sum\limits_{S \in \Theta} P_{Z}(S) \sum\limits_{A \subseteq S, |A|\leq m} q_{S}(A) \sum\limits_{i \in A} w_{i} u_{i}} \\ 
    {\text { subject to }} & {\sum\limits_{S \in \Theta} P_{Z}(S) \sum\limits_{A \subseteq S, |A|\leq m : i \in A} q_{S}(A) \geq k_{i}, \forall i \in \mathcal{N}}, \\  
    {}& {\sum\limits_{A \subseteq S : |A|\leq m} q_{S}(A)=1, \forall S \in \Theta}, \\ 
    {} & {q_{S}(A) \in[0,1], \forall A \subseteq S, |A|\leq m, \forall S \in \Theta},
    \end{array}
$}
\end{equation}
where the first constraint is equivalent to the fairness constraints defined in (\ref{eq:fraction}), and the second constraint states that for each availability set $S\in \Theta$, the probability space for choosing $A(t)$ should be complete.

Denote the optimal solution to (\ref{eq:question}) as $\mathbf{q}^* = \{q^*_{S}(A), \forall S \in \Theta, A \subseteq S, |A|\leq m\}$, i.e., the optimal policy pulls $A\subseteq S$ with probability $q^*_S(A)$ when observing an available arm set $S$. We denote by $A^*(t)$ the arms pulled by the optimal policy in round $t$.

However,  $P_{Z}$ and $u_i, \forall i \in \mathcal{N}$ are unknown in advance, and the learning agent can only observe the available arms and the random rewards of the pulled arms. Therefore, the learning agent faces the dilemma between exploration and exploitation, i.e., in each round, the agent can either do exploration (acquiring information to estimate the mean reward of each arm) or exploitation (accumulating rewards as many as possible). The quality of the agent’s policy is measured by the \emph{time-averaged regret}, which is the performance loss caused by not always performing the optimal actions.
Considering the stochastic availability of each arm, we define the time-averaged regret as follows:
\begin{equation}\label{eq:regret}
\resizebox{.9\hsize}{!}{$\mathcal{R}(T) := \mathbb{E}\left[\frac{1}{T} \sum_{t=0}^{T-1} \left(\sum_{i \in A^*(t)} w_{i} X_{i}(t) - \sum_{i \in A(t)} w_{i} X_{i}(t)\right)\right]$.}
\end{equation}
% Bingshan Hu, However, in practice, we may not know all the information required and there are some challenges to design an effective and efficient learning algorithm.

% However, in practice, there are following challenges in designing and evaluating an efficient algorithm to solve CSMAB-F.

% \begin{itemize}
%     \item The first challenge is faced by all the stochastic MAB problems, i.e., how to make a good balance between exploration (acquire knowledge) and exploitation (achieve a high cumulative reward). Since the learning agent does not know the mean reward of each arm, she needs to do explorations (pull all the arms at least for a certain number of times) to make the estimation of the mean reward close to the true mean reward with high probability. Meanwhile, if the learning agent pulls the sub-optimal arms too much, it will not be possible to achieve a high cumulative reward.
    
    
%     %reward for each arm $u_i, \forall i \in \mathcal{N}$ is not a prior knowledge, 
%     %the algorithm cannot achieve high rewards~(i.e., exploitation) without acquire enough knowledge about $u_i, \forall i \in \mathcal{N}$~(i.e., exploration), but too much exploration can affect the algorithm achieving higher rewards. 


%     \item The fairness constraints bring another dimension of difficulty. Due to the stochastic availability and the fact that no more than $m$ arms can be pulled simultaneously, there will always be some arms that have not been pulled enough times. Therefore, to satisfy the fairness constraints, some new techniques need to be introduced.
    
%     \item The stochastic availability (the set of available arms may vary in each round $t$) introduces a challenge of the performance evaluation. Since the best arm (the arm with the highest mean reward in set $\mathcal{N}$) may not always be available, i.e., for some round $t$, the best arm is not in $Z(t)$,  the performance of the learning algorithm cannot be evaluated in the same way as in the classic setting. In the classic setting, the performance of the agent's choice is always compared to the best arm and this best arm is fixed during all these $T$ rounds. While in the problem setting of our work, it is unfair if we reuse the same way. Instead, a more reasonable way is to compare the performance of the agent's choice to the best arm that is available, i.e., the best arm in set $Z(t)$. 
    
    
%     %with the highest mean rewards. %but to be compared with the best available actions.
    
%     %there are some arms unavailable to pull in each round, the performance of the algorithm cannot be evaluated in the same way as in the classic setting, but to be compared with the best available actions.
    
    

    
%     %The algorithm needs to record the under-pulled arms and makes up for them in the following rounds.
% \end{itemize}

% % Bingshan has not revised the following paragraph

==> Thompson Sampling for Combinatorial Semi-bandits with Sleeping Arms and Long-Term Fairness Constraints/4-Algorithm.tex <==
\section{Thompson Sampling with Beta Priors and Bernoulli Likelihoods for CSMAB-F (TSCSF-B)}\label{sec:algorithms}

% Bingshan has finished the revise  ******** {

The key challenges to design an effective and efficient algorithm to solve the CSMAB-F problem can be twofold. First, the algorithm should well balance the exploration and exploitation in order to achieve a low time-averaged regret. Second, the algorithm should make a good balance between satisfying the fairness constraints and accumulating more rewards.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[h]
\caption{Thompson Sampling with Beta Priors and Bernoulli Likelihoods for CSMAB-F (TSCSF-B)} \label{alg:CombTS1}
\begin{algorithmic}[1]
  \REQUIRE Arm set $\mathcal{N}$, combinatorial constraint $m$, fairness constraint $\mathbf{k}$, time horizon $T$ and queue weight $\eta$.
  \STATE \textbf{Initialization}: 
  %$h_i(0) = 0$, 
  $Q_i(0) = 0$, $\alpha_i(0) = \beta_i(0) = 1$, $\forall i \in \mathcal{N}$;
  \FOR{$t=0, \ldots, T-1$}
  \STATE Observe the available arm set $Z(t)$;
  \STATE For each arm $i\in Z(t)$, draw a sample $\theta_i \sim \text{Beta}(\alpha_i(t), \beta_i(t))$;
  \STATE Pull arms ${A}(t)$ according to (\ref{eq:solution});
  \STATE Observe rewards $X_i, \forall i \in {A}(t)$;
  \STATE Update $Q_i(t+1)$ based on (\ref{eq:updateQ});
  \FORALL{$i \in {A}(t)$}
  \STATE Update $\alpha_{i}(t)$ and $\beta_{i}(t)$ based on (\ref{eq:updatebeta});
  \ENDFOR
  \ENDFOR
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To address the first challenge, we adopt the Thompson sampling technique with beta priors and Bernoulli likelihoods to achieve the tradeoff between the exploration and exploitation. The main idea is to assume a beta prior distribution with the shape parameters $\alpha_{i}(t)$ and $\beta_{i}(t)$ (i.e., ${\rm Beta}(\alpha_{i}(t),\beta_{i}(t))$) on the mean reward of each arm $u_i$. 
Initially, we let $\alpha_{i}(0)=\beta_{i}(0)=1$, since we have no knowledge about each $u_i$ and ${\rm Beta}(1,1)$ is a uniform distribution in $[0,1]$. Then, after observing the available arms $Z(t)$, we draw a sample $\theta_i(t)$ from ${\rm Beta}(\alpha_{i}(t),\beta_{i}(t))$ as an estimate for $u_i, \forall i \in Z(t)$, and pull arms $A(t)$ according to (\ref{eq:solution}) as discussed later. The arms in $A(t)$ return rewards $X_i(t), \forall i \in A(t)$, which are used to update the beta distributions based on Bayes rules and Bernoulli likelihood for all arms in $A(t)$:
\begin{equation}\label{eq:updatebeta}
\begin{aligned}
  &\alpha_i(t+1) = \alpha_i(t) + X_i(t),\\
  &\beta_i(t+1) = \beta_i(t) + 1 - X_i(t).
\end{aligned}
\end{equation}
After a number of rounds, we are able to see that the mean of the posterior beta distributions will converge to the true mean of the reward distributions.
% Before presenting our proposed algorithm, we will introduce briefly how the standard TS algorithm works. %TS-based algorithms can be categorized into the family of  randomized algorithms. 
% The basic idea is to use the random posterior samples. The learning algorithm first assumes a prior distribution over the mean reward of each arm. At the beginning of each round, for each arm, a random sample $\theta_i(t)$ is drawn from the posterior distribution. Then the agent pulls the arm with the highest posterior sample value.
% After observing the random reward, the posterior distribution of the pulled arm will be updated based on Bayes's rule. After a certain number of rounds, we are able to see that the mean of the posterior distribution will concentrate on the true mean of the reward distribution. However, there are only a few
% theoretical guarantees for the variants of MAB problems and so far, there is no TS algorithm devised for CSMAB-F problems. Therefore, it is desirable to design and derive TS algorithms and theoretical guarantees for CSMAB-F.

The virtual queue technique~\cite{li2019combinatorial,neely2010stochastic} can be used to ensure that the fairness constraints are satisfied. The high-level idea  behind the design is to establish a time-varying queue $Q_i(t)$ to record the number of times that arm $i$ has failed to meet the fairness. Initially, we set $Q_i(0) = 0$ for all $i \in \mathcal{N}$. For the ease of presentation, let $d_i(t) := \mathbf{1}[i \in {A}(t)]$ be a binary random variable indicating that whether arm $i$ is pulled or not in round $t$. Then for each arm $i \in \mathcal{N}$, we can use the following way to maintain the queue:
\begin{equation}\label{eq:updateQ}
  Q_i(t) = \max \left\{t \cdot k_i - \sum_{\tau=0}^{t-1} d_i(t), \ 0 \right\}.
\end{equation}
Intuitively, the length of the virtual queue for arm $i$ increases $k_i$ if the arm is not pulled in  round $t$.  Therefore, arms with longer queues are more unfair and will be given a higher priority to be pulled in future rounds. Note that our queue evolution is slightly different from \cite{li2019combinatorial} to avoid the rounding error accumulation issue.

To further balance the fairness and the reward, we introduce another parameter $\eta$ as a tradeoff between the reward and the virtual queue lengths. Then, in each round $t$, the learning agent pulls arms $A(t)$ as follows:

%On the other hand, we want to pull arms with higher estimated mean rewards. Let $\theta_i$ be the estimated mean reward sampled from the prior distribution for arm $i$. To balance the aforementioned two objectives,  we defined the policy $A(t)$ as follows:

\begin{equation}\label{eq:solution}
    A(t) \in \underset{A \subseteq {Z}(t), |A| \leq m}{\operatorname{argmax}} \sum_{i \in A}\left(\frac{1}{\eta} Q_{i}(t) +  w_{i} \theta_i(t)\right).
\end{equation}
Note that different from LFG, we weigh $Q_i(t)$ with $\frac{1}{\eta}$ in (\ref{eq:solution}) rather than weighing $\theta_i(t)$ with $\eta$. The advantage is that we can simply let $\eta \rightarrow \infty$ to neglect virtual queues, so the algorithm can be adapted to CSMAB easily. The whole process of the TSCSF-B algorithm is shown in Alg.~\ref{alg:CombTS1}.

% Bingshan has finished the revise  ******** }


%Next, we introduce two TS-based algorithms using the Beta priors and the Gaussian priors, respectively. The main difference between the two algorithms is that they use different prior distributions and different likelihood functions to estimate the mean rewards. Beta distribution is defined on the interval $[0,1]$ with two positive parameters $\alpha$ and $\beta$ to control its shape, while Gaussian distribution is defined on the interval $(-\infty,\infty)$ with parameter $\hat{u}$ as the mean of the distribution and $\sigma$ as the standard deviation. 
% Bingshan suggests to revise the following part as
%Thus, it is easy to see that Gaussian distribution is natural to support $X_i(t) \in [-\infty,\infty]$ but with a high uncertain $\theta_i$. On the other hand, Beta distributions only support $X_i(t) \in [0,1]$ but the posterior sample $\theta_i$ is less uncertain, which is always within $[0,1]$.
% New version
% Therefore, it is easy to see that Gaussian distribution is natural to support $X_i(t) \in [-\infty,\infty]$ while Beta distribution can only support $X_i(t) \in [0,1]$. For both algorithms, we define $h_i(t)$ as the number of times that arm $i$ has been pulled at the beginning of round $t$.


%For each arm $i$, $X_i(t)$’s are i.i.d. with mean $u_i$, and $Y_i(t)$ is a Bernoulli random variable with mean $X_i(t)$. Thus $Y_i(t)$’s are also i.i.d. with mean $u_i$. Therefore, it is easy to show that any expected regret bounds produced for Algorithm \ref{alg:CombTS1} will also hold for this extension~\cite{agrawal2012analysis}.

%the Beta prior for each arm $i$ by generating a Bernoulli random variable $Y_i(t)$ with mean $X_i(t)$.



==> Thompson Sampling for Combinatorial Semi-bandits with Sleeping Arms and Long-Term Fairness Constraints/5-Results.tex <==
\section{Results and Proofs}\label{sec:results}
\subsection{Fairness Satisfaction}
% Recall that the virtual queue system incorporated in the proposed algorithms records the ``under-played" arms, i.e., if the fairness of an arm is not satisfied, the virtual queue for that arm is not empty. Therefore, to measure whether the proposed algorithms can achieve fairness constraints, we can check whether the virtual queues are \emph{mean rate stable}~\cite{li2019combinatorial,neely2010stochastic}:
% \begin{equation*}
%     \lim _{T \rightarrow \infty} \frac{\mathbb{E}\left[\sum_{i=1}^{N} Q_{i}(T)\right]}{T}=0,
% \end{equation*}
% where given enough time, all the virtual queues in the last rounds should be empty.
% The mean rate stable property can be proved by Theorem \ref{thm:feasbility}.
%can satisfy the fairness constraints defined in (\ref{eq:fraction}),
\begin{theorem}\label{thm:feasbility}
For any fixed and finite $\eta>0$, when $T$ is long enough and the fairness constraint vector $\mathbf{k}$ is feasible, the proposed TSCSF-B algorithm satisfies the long-term fairness constraints defined in (\ref{eq:fraction}).
\end{theorem}
\begin{proof}[Proof Sketch]
The main idea to prove Theorem \ref{thm:feasbility} is to prove the virtual queue for each arm is stable when $\mathbf{k}$ is feasible and $T$ is long enough for any fixed and finite $\eta>0$.  The proof is based on Lyapunov-drift analysis~\cite{neely2010stochastic}. Since it is not our main contribution and it follows similar lines to the proof of Theorem 1 in \cite{li2019combinatorial},  we omit the proof. Interested readers are referred to \cite{li2019combinatorial}.
\end{proof}
\begin{remark}
The long-term fairness constraints does not require arms to be pulled for a certain number of times in each round but by the end of the time horizon. Theorem \ref{thm:feasbility} states that the fairness constraints can always be satisfied by TSCSF-B as long as $\eta$ is finite and $T$ is long enough. A higher $\eta$ may require a longer time for the fairness constraints to be satisfied~(see Sec.~\ref{sec:evaluation}).
%This give us a hint to choose appropriate $\eta$ in practice. If the application has a loose fairness requirement, we can enlarge $\eta$ to achieve more rewards.
\end{remark}


\subsection{Regret Bounds}
% We define the time-average regret of TSCSF-B as
% \begin{equation*}
%     \begin{aligned}
%     R_{\mathrm{TSCSF-B}}(T)
%     &=\frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i \in A^{*}(t)} w_{i} u_{i}-\sum_{i \in A(t)} w_{i} u_{i}\right] \\
%     &=\frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E}\left[\underbrace{\sum_{i=1}^{N} w_{i} u_{i} d_{i}^{*}(t)-\sum_{i=1}^{N} w_{i} u_{i} d_{i}(t)}_{\Delta r_{(t)}}\right].
%     \end{aligned}
% \end{equation*}
\begin{theorem}\label{thm:regret}
For any fixed $T>1, \eta>0, w_{\max} > 0$ and $m \in (0,N]$, the time-averaged regret of TSCSF-B is upper bounded by
\begin{equation*}
   \frac{N}{2\eta} + \frac{4w_{\max}\sqrt{mNT\ln T} + 2.51 w_{\max} N }{T}.
\end{equation*}
\end{theorem}
\begin{proof}[Proof Sketch]\label{skpf:regret1}
We only provide a sketch of proof here, and the detailed proof can be found in Appendix. The optimal policy for CSMAB-F is a randomized algorithm defined in Sec.~\ref{sec:problem}, while the optimal policies for classic MAB problems are deterministic. We follow the basic idea in \cite{li2019combinatorial} to convert the regret bound between the randomized optimal policy and TSCSF-B~(i.e., regret) by the regret bound between a deterministic oracle and TSCSF-B. The deterministic oracle also knows the mean reward for each arm, and can achieve more rewards than the optimal policy by sacrificing fairness constraints a bit. Denote the arms pulled by the oracle in round $t$ as $A^{\prime}(t)$, which is defined by
\begin{equation*}
    A^{\prime}(t) \in \underset{A \subseteq Z(t), |A| \leq m}{\operatorname{argmax}} \sum_{i \in A}\left(\frac{1}{\eta} Q_{i}(t) +  w_{i} u_{i}(t)\right).
\end{equation*}
Then, we can prove that the time-averaged regret defined in (\ref{eq:regret}) is bounded by
\begin{equation}\label{eq:astar}
\resizebox{.9\hsize}{!}{$
\frac{N}{2 \eta}+\frac{1}{T} \left(\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i \in A(t)} w_{i}\left(\theta_{i}(t)-u_{i}\right)\right] + \sum_{t=0}^{T-1}\mathbb{E}\left[\sum_{i \in A^{\prime}(t)} w_{i}\left(u_{i}-\theta_{i}(t)\right)\right]}_{C}\right)$,}
\end{equation}
where the first term $\frac{N}{2\eta}$ is due to the queuing system, and the second part $C$ is due to the exploration and exploitation.

Next, we define two events and their complementary events for each arm $i$ to decompose $C$. Let $\gamma_i(t) := \sqrt{\frac{2\ln T}{h_i(t)}}$, where $h_i(t)$ is the number of times that arm $i$ has been pulled at the beginning of round $t$. Then for each arm $i\in \mathcal{N}$, the two events $\mathcal{J}_i(t)$ and $\mathcal{K}_i(t)$ are defined as follows:
\begin{equation*}
\begin{aligned}
   &\mathcal{J}_i(t) := \{\theta_i(t)  - u_i > 2\gamma_i(t) \},\\
   &\mathcal{K}_i(t) := \{u_i - \theta_i(t)> 2\gamma_i(t) \},
\end{aligned}
\end{equation*}
and let $\overline{\mathcal{J}_i(t)}$ and $\overline{\mathcal{K}_i(t)}$ be the complementary events for  $\mathcal{J}_i(t)$ and $\mathcal{K}_i(t)$, respectively.
Notice that both $\mathcal{J}_i(t)$ and $\mathcal{K}_i(t)$ are low-probability events after a number of rounds.
%Let $\overline{\mathcal{J}_i(t)}$ and $\overline{\mathcal{K}_i(t)}$ be the complementary events for events $\mathcal{J}_i(t)$ and $\mathcal{K}_i(t)$, respectively.

With the events defined above, we can decompose $C$ as
\begin{equation*}
\resizebox{1.0\hsize}{!}{$
\begin{aligned}
     &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i\in A(t)} w_{i}\left(\theta_{i}(t)-u_{i}\right) \mathbf{1}[\mathcal{J}_i(t)] \right]}_{B_1}
     + \underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i\in A(t)} w_{i}\left(\theta_{i}(t)-u_{i}\right) \mathbf{1}[\overline{\mathcal{J}_i(t)}] \right]}_{B_2}\\
     + &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i\in A^\prime(t)} w_{i}\left(\theta_{i}(t)-u_{i}\right) \mathbf{1}\left[\mathcal{K}_i(t)\right]\right]}_{B_3}
     + \underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i\in A^\prime (t)} w_{i}\left(\theta_{i}(t)-u_{i}\right)  \mathbf{1}\left[\overline{\mathcal{K}_i(t)}\right] \right]}_{B_4}.
\end{aligned}$}
\end{equation*}

Using the relationship between the summation and integration, we can bound $B_2$ and $B_4$ by $4w_{\max} \sqrt{mNT\ln T} + w_{\max}N$.

Bounding $B_1$ and $B_3$ is the main theoretical contribution of our work and is not trivial. Since $\mathcal{J}_i(t)$ and $\mathcal{K}_i(t)$ are low-probability events, the total times they can happen are a constant value on expectation. Therefore, to bound $B_1$ and $B_3$,  the basic idea is to obtain the bounds for $\Pr(\mathcal{J}_i(t))$ and $\Pr(\mathcal{K}_i(t))$. Currently, there is no existing work giving the bounds for $\Pr(\mathcal{J}_i(t))$ and $\Pr(\mathcal{K}_i(t))$, and we prove that $\Pr(\mathcal{J}_i(t))$ and $\Pr(\mathcal{K}_i(t))$ are bounded by $\left(\frac{1}{T^2}+\frac{1}{T^{32}}\right)$ and $\left(\frac{1}{T^8} + \frac{1}{T^{32}} \right)$, respectively. Then, it is straightforward to bound $B_1$ and $B_3$ by $2.51w_{\max}N$.

%The detailed proof can be referred to Appendix \ref{sec:thm52}.
\end{proof}
\begin{remark}
Comparing with the time-averaged regret bound for LFG~\cite{li2019combinatorial},  we have the same first term $\frac{N}{2\eta}$, as we adopt the virtual queue system to satisfy the fairness constraints. On the other hand, the second part of our regret bound, which is also the first problem-independent regret bound for CSMAB problems, has lower coefficients than that of LFG. Specifically, the coefficient for the time-dependent term (i.e., $\sqrt{mNT\ln T}$) is $4$ in our bound, smaller than $2\sqrt{6}$ in that of LFG, and the time-independent term (i.e., $w_{\max}N$) has a coefficient $2.51$ in our bound, which is also less than $5.11$ in the bound of LFG.
%Although our proposed algorithm has a bit higher coefficients for time-independent component (i.e., $w_{\max} N$), the effect can be neglected if the time horizon $T$ is larger than $N$.

If we let $\eta \rightarrow \infty$, the algorithm only focuses on CSMAB problems, and the bound boils down to the first problem-independent bound of TS-based algorithms for CSMAB problems, which matches the lower bound proposed in \cite{kveton2015tight}.
\end{remark}
\begin{corollary}\label{cr:1}
For any fixed $m \in (0,N]$ and $\eta \geq \sqrt{\frac{NT}{m\ln T}}$, when $T \geq N$, the time-averaged regret of TSCSF-B is upper bounded by $\widetilde{O}\left(\frac{\sqrt{mNT}}{T}\right).$
\end{corollary}
\begin{remark}
The reason we let $\eta \geq \sqrt{\frac{NT}{m\ln T}}$ for a given $T$ is to control the first term to have a consistent or lower order than the second term. However, in practice, we need to tune $\eta$ according to $T$ such that both fairness constraints and high rewards can be achieved.
%the bound can become much tighter, otherwise
\end{remark} 

==> Thompson Sampling for Combinatorial Semi-bandits with Sleeping Arms and Long-Term Fairness Constraints/6-Proof.tex <==
\section{Proof of Regret Bounds}
%In this section, we prove Theorem \ref{thm:regret} and Theorem \ref{thm:regret2}. The proofs of Theorem \ref{thm:regret} and Theorem \ref{thm:regret2} are similar but they use different concentration inequalities in the end of the analysis.
\subsection{Notations}
Recall $\hat{u}_{i}(t) := \frac{\alpha_{i}(t)-1}{h_{i}(t)}=\frac{1}{h_{i}(t)} \sum\limits_{\tau: \tau<t, i \in A(\tau)} X_{i}(t)$ is the empirical mean of arm $i$ until the beginning of round $t$.  Therefore, we have $\alpha_i(t) -1  = \hat{u}_{i}(t) h_i(t) = \hat{u}_{i}(t) (\alpha_{i}(t) + \beta_i(t)-2)$. 

For each arm $i\in \mathcal{N}$, we have three events $\mathcal{J}_i(t)$, $\mathcal{K}_i(t)$ and $\mathcal{H}_i(t)$ defined as follows:
\begin{equation*}
\begin{aligned}
   &\mathcal{J}_i(t) := \{\theta_i(t)  - u_i > 2\gamma_i(t) \},\\
   &\mathcal{K}_i(t) := \{u_i - \theta_i(t)> 2\varepsilon_i(t) \},\\
   &\mathcal{K}_i(t) := \{u_i - \theta_i(t)> 2\gamma_i(t).
\end{aligned}
\end{equation*}
where $\gamma_i(t) := \sqrt{\frac{2\ln T}{h_i(t)}}, \varepsilon_i(t) := \sqrt{\frac{2\ln t}{h_i(t)}}$. 


\subsection{Proof of Theorem \ref{thm:regret}}\label{sec:thm52}
To prove Theorem \ref{thm:regret}, we first introduce the following lemmas with the proofs in Sec.~\ref{sec:pfoflemmas}.

\begin{lemma}\label{lm:main}
\cite{li2019combinatorial}. Then the time-average regret of TSCSF-B or TSCSF-G can be bounded by
\begin{equation}\label{eq:astar}
\small
\begin{aligned}
\frac{N}{2 \eta}+\frac{1}{T} \left(\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i \in A(t)} w_{i}\left(\theta_{i}(t)-u_{i}\right)\right]}_{C_1} +  \underbrace{\sum_{t=0}^{T-1}\mathbb{E}\left[\sum_{i \in A^{\prime}(t)} w_{i}\left(u_{i}-\theta_{i}(t)\right)\right]}_{C_2}\right).
\end{aligned}
\end{equation}
\end{lemma}



\begin{lemma}\label{lm:ft}
For all $i \in \mathcal{N}, t \leq T$, the probability that event ${\mathcal{J}_i(t)}$ happens is upper bounded as follows:
\begin{equation*}
    \Pr\left(\mathcal{J}_i(t)\right) \leq \frac{1}{T} + \frac{1}{T^4},
\end{equation*}
\end{lemma}

\begin{lemma}\label{lm:kt}
For all $i \in \mathcal{N}, h_i(t) \geq 4$ and $t \leq T$, the probability that event ${\mathcal{K}_i(t)}$ happens is upper bounded as follows:
\begin{equation*}
    \Pr\left(\mathcal{K}_i(t)\right) \leq \frac{1}{t^2} + \frac{1}{t^4}.
\end{equation*}
\end{lemma}

\begin{proof}
First, by Lemma \ref{lm:main} we have $R_{\mathrm{TSCSF-B}}(T)$ bounded by
(\ref{eq:astar}).

\paragraph{Bound $C_1$}
Define event $\overline{\mathcal{J}_i(t)}$ is the complementary event of $\mathcal{J}_i(t)$ as follows:
\begin{equation*}
    \overline{\mathcal{J}_i(t)} := \{\theta_i(t) - u_i \leq 2\gamma_i(t) \}.
\end{equation*}
Then, we can decompose $C_1$ as
\begin{equation*}\label{eq:c1}
\begin{aligned}
    &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}[\mathcal{J}_i(t)] \right]}_{B_1} \\
    + &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}[\overline{\mathcal{J}_i(t)}] \right]}_{B_2}.
\end{aligned}
\end{equation*}
Since $\theta_{i}(t)-u_{i}\leq 1, d_{i}(t)\leq 1$, $B_1$ is therefore bounded by
\begin{equation*}\label{eq:b2}
\begin{aligned}
    \sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i} \mathbf{1}[{\mathcal{J}_i(t)}] \right] \leq & w_{\max}\sum_{i=1}^{N} \sum_{t=0}^{T-1} \Pr\left({\mathcal{J}_i(t)}\right)\\
    \leq & w_{\max}\sum_{i=1}^{N} \sum_{t=0}^{T-1} \left(\frac{1}{T}+\frac{1}{T^4}\right)\\
    \leq & 2 w_{\max} N,
\end{aligned}
\end{equation*}
where the second inequality is due to Lemma \ref{lm:ft}.


Next, we show how to bound $B_2$. Let $\tau_{i}(a)$ be the round where arm $i$ is played for the $a$-th time, i.e., $h_{i}(\tau_{i}(a)) = a-1$.
$B_2$ can be bounded as follows:
\begin{equation}\label{eq:B1}
\begin{aligned}
    &\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}\left[\overline{\mathcal{J}_i(t)}\right] \right]\\
    =&\sum_{i=1}^{N} \mathbb{E}\left[\sum_{a=1}^{h_{i}(T-1)} \sum_{\tau_i(a)}^{\tau_{i}(a+1)-1} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}\left[\overline{\mathcal{J}_i(t)}\right]\right]\\
    \leq& \sum_{i=1}^{N} \mathbb{E}\left[w_{1} + \sum_{a=2}^{h_{i}(T-1)} \sum_{\tau_i(a)}^{\tau_{i}(a+1)-1} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}\left[\overline{\mathcal{J}_i(t)}\right]\right]\\
    \leq& w_{\max}\sum_{i=1}^{N} \mathbb{E}\left[1 + 2 \sum_{a=2}^{h_{i}(T-1)} \sum_{\tau_i(a)}^{\tau_{i}(a+1)-1} \gamma_i(t) d_{i}(t) \right]\\
    =& w_{\max}N + 2w_{\max}\sum_{i=1}^{N} \mathbb{E}\left[\sum_{a=2}^{h_{i}(T-1)} \gamma_i(\tau_i(a))\right].
\end{aligned}
\end{equation}
The last term in (\ref{eq:B1}) can be further written as follows:
\begin{equation*}\label{eq:2wb}
    \begin{aligned}
    & 2w_{\max}\sum_{i=1}^{N}  \mathbb{E}\left[ \sum_{a = 2}^{h_i(T-1)} \gamma_i(\tau_i(a))\right]\\ 
    =& 2w_{\max}\sum_{i=1}^{N} \mathbb{E}\left[ \sum_{a = 2}^{h_i(T-1)} \sqrt{\frac{2\ln T}{a-1}}\right]\\
    =& 2w_{\max} \sqrt{2\ln T} \sum_{i=1}^{N}  \mathbb{E}\left[ \sum_{a = 2}^{h_i(T-1)} \sqrt{\frac{1}{a-1}}\right] \\
    {\leq} & 2w_{\max} \sqrt{2\ln T} \sum_{i=1}^{N}  \mathbb{E}\left[ 1 + \int_{1}^{h_i(T-1)} \sqrt{\frac{1}{x}} dx \right]\\
     {\leq}& 2w_{\max} \sqrt{2\ln T} \sum_{i=1}^{N}  \mathbb{E}\left[ \sqrt{h_i(T-1)}\right]\\
     {\leq} & 2w_{\max} \sqrt{2\ln T} \sum_{i=1}^{N}   \sqrt{\mathbb{E}\left[h_i(T-1)\right]},
    \end{aligned}
\end{equation*}
where the last inequality is due to Jensen's inequality. Also by Jensen's inequality, we have
\begin{equation*}
    \frac{1}{N}\sum\limits_{i=1}^{N}   \sqrt{\mathbb{E}\left[h_i(T-1)\right]} \leq \sqrt{\frac{1}{N} \sum\limits_{i=1}^{N}\mathbb{E}\left[h_i(T-1)\right]}.
\end{equation*}
Therefore, we can bound $\sum\limits_{i=1}^{N}   \sqrt{\mathbb{E}\left[h_i(T-1)\right]}$ by
\begin{equation*}\label{eq:lb1t}
\begin{aligned}
     \sqrt{N \sum\limits_{i=1}^{N}\mathbb{E}\left[h_i(T-1)\right]}
    \leq \sqrt{NTm},
\end{aligned}
\end{equation*}
where the inequality is due to the fact that at most $m$ arms are selected in each round.
Therefore, we have $B_2$ bounded by
\begin{equation*}\label{eq"b1bound}
    2w_{\max} \sqrt{2mNT\ln T} + w_{\max}N.
\end{equation*}


Combining $B_1$ and $B_2$ gives
\begin{equation*}
    C_1 \leq 2w_{\max}\sqrt{2mNT\ln T} +  3w_{\max}N.
\end{equation*}

\paragraph{Bound $C_2$} 
Define an event $\overline{\mathcal{K}_i(t)}$ as the complementary event of $\mathcal{K}_i(t)$:
\begin{equation*}
    \overline{\mathcal{K}_i(t)} := \{u_i - \theta_i(t) \leq 2\varepsilon_i(t)\}.
\end{equation*}
$C_2$ can be decomposed by
\begin{equation*}\label{eq:c2}
\begin{aligned}
    &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d^\prime_{i}(t) \mathbf{1}\left[\mathcal{K}_i(t)\right]\right]}_{B_3} \\
    + &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d^\prime_{i}(t) \mathbf{1}\left[\overline{\mathcal{K}_i(t)}\right] \right]}_{B_4}.
\end{aligned}
\end{equation*}

Let $\tau^\prime_{i}(a)$ be the round where arm $i$ is played for the $a$-th time by policy $A^\prime(t)$, i.e., $h^\prime_{i}(\tau^\prime_{i}(a)) = a - 1$. Since $\theta_{i}(t)-u_{i}\leq 1$, we can write $B_3$ as follows:
\begin{equation*}\label{eq:b4}
\begin{aligned}
    B_4 \leq& w_{\max} \sum_{i=1}^N \mathbb{E}\left[\sum_{t=1}^{T-1} d^\prime_{i}(t) \mathbf{1}\left[\overline{\mathcal{K}_i(t)}\right] \right] \\
    =& w_{\max} \sum_{i=1}^N \mathbb{E}\left[\sum_{a=1}^{h_i^\prime(T-1)} \mathbf{1}\left[\overline{\mathcal{K}_i(\tau^\prime_{i}(a))}\right] \right] \\
    \leq & w_{\max} \sum_{i=1}^N \mathbb{E}\left[\sum_{a=1}^{3}1 + \sum_{a=4}^{h_i^\prime(T-1)} \mathbf{1}\left[\overline{\mathcal{K}_i(\tau^\prime_{i}(a))}\right] \right]\\
    \leq & 3w_{\max}N +  w_{\max} \sum_{i=1}^N \sum_{a=4}^{\infty} \Pr\left(\overline{\mathcal{K}_i(\tau^\prime_{i}(a))}\right)\\
    \stackrel{(\rm a)}{=} & 3 w_{\max} N + w_{\max} \sum_{i=1}^N \sum_{a=4}^{\infty} \left(\frac{1}{(\tau^\prime_{i}(a))^2} + \frac{1}{(\tau^\prime_{i}(a))^4} \right)\\
    \leq & 3 w_{\max} N + w_{\max} \sum_{i=1}^N \sum_{t=1}^{\infty} \left(\frac{1}{t^2} + \frac{1}{t^4} \right)\\
    \leq & 3 w_{\max} N + w_{\max} \sum_{i=1}^N  \left(\frac{\pi^2}{6} + \frac{\pi^4}{90} \right)\\
    \leq & 5.73w_{\max}N.
\end{aligned}
\end{equation*}
where (a) is due to Lemma \ref{lm:kt}.

$B_4$ can be bounded in a similar way as $B_2$:
\begin{equation*}\label{eq:b3}
\begin{aligned}
    B_3 \leq& w_{\max}N + 2w_{\max} \sum_{i=1}^{N} \mathbb{E}\left[\sum_{a=2}^{h^\prime_i(T-1)}\sqrt{\frac{2 \ln t}{a-1}} \right]\\
    \leq & w_{\max}N  + 2w_{\max} \sqrt{\ln T} \sum_{i=1}^{N} \mathbb{E}\left[\sum_{a=2}^{h^\prime_i(T-1)}\sqrt{\frac{1}{a-1}} \right]\\
    \leq & 2w_{\max} \sqrt{2mNT\ln T} + w_{\max}N .
\end{aligned}
\end{equation*}

Therefore, we have $C_2$ bounded by
\begin{equation*}\label{eq:c21}
    2w_{\max}\sqrt{2mNT\ln T} + 6.73 w_{\max}N.
\end{equation*}
Theorem \ref{thm:regret} is proved by combining the bound of $C_1$ and $C_2$.
\end{proof}

\subsection{Proof of Theorem \ref{thm:regret2}}\label{pf:regret2}
To bound Theorem \ref{thm:regret2}, we introduce the following Lemma with a proof in Sec.~\ref{sec:pfoflemmas}:
\begin{lemma}\label{lm:gs}
For all $i \in \mathcal{N}, h_i(t)>0$ and $t \leq T$, the probabilities that event ${\mathcal{J}_i(t)}$ happens and event ${\mathcal{H}_i(t)}$ happens are upper bounded as follows:
\begin{equation*}
\begin{aligned}
    &\Pr\left({\mathcal{J}_i(t)}\right) \leq \frac{1}{2T} + \frac{1}{T^4},\\
    &\Pr\left({\mathcal{H}_i(t)}\right) \leq \frac{1}{2T} + \frac{1}{T^4}.
\end{aligned}
\end{equation*}
\end{lemma}

\begin{proof}
Similar to the proof of Theorem \ref{thm:regret}, we first use Lemma \ref{lm:main} to have $R_{\mathrm{TSCSF-G}}(T)$ bounded by
\begin{equation}
\begin{aligned}
\frac{N}{2 \eta}+\frac{1}{T} \left(C_1 + C_2\right).
\end{aligned}
\end{equation}

Then we can decompose $C_1$ as follows:
\begin{equation}\label{eq:c3}
\begin{aligned}
    &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}[\mathcal{J}_i(t)] \right]}_{B_5} \\
    + &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d_{i}(t) \mathbf{1}[\overline{\mathcal{J}_i(t)}] \right]}_{B_6}.
\end{aligned}
\end{equation}
We can bound $B_5$ by Lemma \ref{lm:gs} as follows:
\begin{equation}\label{eq:b6}
\begin{aligned}
    B_6 \leq& w_{\max} \sum_{i=1}^{N} \mathbb{E}\left[\sum_{t=0}^{T-1} \mathbf{1}[{{\mathcal{J}_i(t)}}] \right]\\
    =& w_{\max} \sum_{i=1}^{N} \sum_{t=0}^{T-1} \Pr\left({{\mathcal{J}_i(t)}}\right)\\
    \leq& w_{\max} \sum_{i=1}^{N} \sum_{t=0}^{T-1} \left(\frac{1}{2T}+\frac{1}{T^4}\right)\\
    \leq& 1.5 w_{\max} N.
\end{aligned}
\end{equation}


On the other hand, we can bound $B_6$ in the same way as $B_2$ by
\begin{equation}\label{eq:b5}
    2w_{\max} \sqrt{2mNT\ln T} + w_{\max}N.
\end{equation}


Substituting (\ref{eq:b6}) and (\ref{eq:b5}) into (\ref{eq:c3}), we have $C_1$ bounded by
\begin{equation*}
    2w_{\max}\sqrt{2mNT\ln T} + 2.5 w_{\max} N.
\end{equation*}

Define event $\overline{\mathcal{H}_i(t)}$ as the complementary event of $\mathcal{H}_i(t)$:
\begin{equation*}
    \overline{\mathcal{H}_i(t)} = \{\theta_i(t)-u_i\leq 2\gamma_i(t) \}.
\end{equation*}

$C_2$ can be decomposed by whether events $\mathcal{H}_i(t)$ and $\overline{\mathcal{H}_i(t)}$ happen as follows:

\begin{equation*}\label{eq:c2}
\begin{aligned}
    &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d^\prime_{i}(t) \mathbf{1}\left[\mathcal{H}_i(t)\right]\right]}_{B_7} \\
    + &\underbrace{\sum_{t=0}^{T-1} \mathbb{E}\left[\sum_{i=1}^{N} w_{i}\left(\theta_{i}(t)-u_{i}\right) d^\prime_{i}(t) \mathbf{1}\left[\overline{\mathcal{H}_i(t)}\right] \right]}_{B_8}.
\end{aligned}
\end{equation*}

We have $B_7$ bounded by $1.5w_{\max}N$ with Lemma \ref{lm:gs}, and $B_8$ bounded by $2w_{\max}\sqrt{2mNT\ln T} + 2.5 w_{\max} N$ with the same steps as bounding $B_1$.
Theorem \ref{thm:regret2} is proved by combining $C_1$ and $C_2$ together.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%proof of lemmas%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemmas}\label{sec:pfoflemmas}

\subsubsection{Proof of Lemma \ref{lm:main}}

\begin{proof}
The proof for Lemma \ref{lm:main} is similar to Theorem 1 in~\cite{li2019combinatorial}. 

Note that the arms selection (defined in (\ref{eq:solution})) is different from LFG~\cite{li2019combinatorial}(we put $\eta$ with the virtual queue), we show that Lemma \ref{lm:main} works for our setting as well.

Following the similar lines in \cite{li2019combinatorial,neely2010stochastic}, we first consider the Lyapunov drift function:
\begin{equation*}
    L(\mathbf{Q}(t)) := \frac{1}{2} \sum_{i=1}^{N} Q_{i}^{2}(t).
\end{equation*}
Recall the regret definition as follows:
\begin{equation*}
\begin{aligned}
    \mathcal{R}(T) &:= \mathbb{E}\left[\frac{1}{T} \sum_{t=0}^{T-1} {\left(\sum_{i \in A^*(t)} w_{i} X_{i}(t) - \sum_{i \in A(t)} w_{i} X_{i}(t)\right)}\right]\\
    & = \frac{1}{T} \sum_{t=0}^{T-1}\mathbb{E}\left[\sum_{i \in A^*(t)} w_{i} u_{i}(t) - \sum_{i \in A(t)} w_{i} u_{i}(t)\right]\\
    & = \frac{1}{T} \sum_{t=0}^{T-1}\mathbb{E}\left[\underbrace{\sum_{i = 1}^N w_{i} u_{i}(t) d^*_i(t)- \sum_{i = 1}^N w_{i} u_{i}(t) d_i(t)}_{\Delta r_i(t)} \right].,
\end{aligned}
\end{equation*}
where $d^*_i(t) = \mathbf{1}\left[i \in A^*_i(t) \right]$ and $d_i(t) = \mathbf{1}\left[i \in A_i(t) \right]$.

Then, the drift-plus-regret is given by
\begin{equation}
\begin{aligned}
    &L(\mathbf{Q}(t+1))-L(\mathbf{Q}(t))+\eta \Delta r_i(t) \\ 
    &=\frac{1}{2} \sum\limits_{i=1}^{N} Q_{i}^{2}(t+1)-\frac{1}{2} \sum\limits_{i=1}^{N} Q_{i}^{2}(t)+\eta \Delta r_i(t) \\ 
    &\stackrel{(\rm a)} {=}\frac{1}{2}\sum\limits_{i=1}^{N}\left(Q_{i}(t)+k_{i}-d_{i}(t)\right)^{2}-\frac{1}{2} \sum\limits_{i=1}^{N} Q_{i}^{2}(t)+\eta \Delta r_i(t) \\ 
    &=\frac{1}{2} \sum\limits_{i=1}^{N}\left(k_{i}-d_{i}(t)\right)^{2}+\sum\limits_{i=1}^{N}\left(k_{i}-d_{i}(t)\right) Q_{i}(t)+\eta \Delta r_i(t) \\ 
    &\stackrel{(\rm b)} {\leq} \frac{N}{2}+\sum\limits_{i=1}^{N} k_{i} Q_{i}(t)-\sum\limits_{i=1}^{N} d_{i}(t) Q_{i}(t)\\
    &+\eta \sum\limits_{i=1}^{N} w_{i} u_{i} d_{i}^{*}(t)-\eta \sum\limits_{i=1}^{N} w_{i} u_{i} d_{i}(t) \\
    &= \frac{N}{2}+\sum\limits_{i=1}^{N}\left(Q_{i}(t)+\eta w_{i} u_{i}\right)\left(d_{i}^{*}(t)-d_{i}(t)\right) \\ 
    &+\sum\limits_{i=1}^{N} Q_{i}(t)\left(k_{i}-d_{i}^{*}(t)\right),
\end{aligned}
\end{equation}
where (a) is due to (\ref{eq:updateQ}), and (b) is due to facts that $k_{i}-d_{i}(t)\leq 1$ and $\Delta r_i(t) > 0$


We can bound the expected drift-plus-regret as
\begin{equation}\label{eq:dpr}
\begin{aligned}
     &\mathbb{E}[L(\mathbf{Q}(t+1))-L(\mathbf{Q}(t))+\eta \Delta r_i(t)]\\ 
     &\leq \frac{N}{2}+\sum\limits_{i=1}^{N} \mathbb{E}\left[\left(Q_{i}(t)+\eta w_{i} u_{i}\right)\left(d_{i}^{*}(t)-d_{i}(t)\right)\right]\\
     &+\sum\limits_{i=1}^{N} \mathbb{E}\left[Q_{i}(t)\left(k_{i}-d_{i}^{*}(t)\right)\right] \\ 
     &\leq \frac{N}{2}+\mathbb{E}[\sum\limits_{i=1}^{N}\left(Q_{i}(t)+\eta w_{i} u_{i}\right)\left(d_{i}^{*}(t)-d_{i}(t)\right)],
\end{aligned}
\end{equation}
where the last inequality is due to $\mathbb{E}\left[d_{i}^{*}(t)\right] \geq k_{i}$.



Summing (\ref{eq:dpr}) for all
$t\in\{0,\ldots,T-1\}$, and
dividing both sides of the inequality by $T\eta$, we have
\begin{equation*}
\begin{aligned}
    &\frac{1}{T \eta} \mathbb{E}[L(\mathbf{Q}(T))-L(\mathbf{Q}(0))]+\frac{1}{T} \sum\limits_{t=0}^{T-1} \mathbb{E}[\Delta r_i(t)] \\ 
    &\leq \frac{N}{2 \eta}+\frac{1}{T} \mathbb{E}[\underbrace{\sum\limits_{i=1}^{N}  \left(\frac{1}{\eta}Q_{i}(t)+ w_{i} u_{i}\right)\left(d_{i}^{*}(t)-d_{i}(t)\right)}_{C(t)}]
\end{aligned}
\end{equation*}

Since $L(Q(T)) \geq 0$ and $L(Q(0)) = 0$, we have 
\begin{equation}\label{eq:regretbound}
    \mathcal{R}(T) = \frac{1}{T} \sum_{t=0}^{T-1} \mathbb{E}[\Delta r_i(t)] \leq \frac{N}{2 \eta}+\frac{1}{\eta T} \sum_{t=0}^{T-1} \mathbb{E}\left[C(t)\right]
\end{equation}



Recall that in each round $t$, the TSCSF-B and TSCSF-G algorithms choose
arms $A(t)$ according to the follows:
\begin{equation*}
    A(t) \in \underset{A \subseteq {Z}(t), |A| \leq m}{\operatorname{argmax}} \sum_{i \in S}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} \theta_{i}(t)\right),
\end{equation*}
and the oracle (see the sketch proof for Theorem \ref{skpf:regret1}) chooses arms $A^\prime (t)$ as follows:
\begin{equation}\label{eq:1eeeeee}
    A^{\prime}(t) \in \underset{A \subseteq Z(t), |A| \leq m}{\operatorname{argmax}} \sum_{i \in A}\left(\frac{1}{\eta}Q_{i}(t)+w_{i} u_{i}(t)\right).
\end{equation}

Therefore, we have
\begin{equation}\label{eq:1eee}
    \sum_{i \in A(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} \theta_{i}(t)\right) \geq \sum_{i \in A^{\prime}(t)}\left(\frac{1}{\eta} Q_{i}(t) + w_{i} \theta_{i}(t)\right)
\end{equation}

$C(t)$ can be bounded as follows:
\begin{equation}\label{eq:ct}
    \begin{aligned}
    C(t)=& \sum_{i=1}^{N}\left(\frac{1}{\eta} Q_{i}(t)+ w_{i} u_{i}\right)\left(d_{i}^{*}(t)-d_{i}(t)\right) \\
    =& \sum_{i \in A^{*}(t)}\left(\frac{1}{\eta} Q_{i}(t)+ w_{i} u_{i}\right)-\sum_{i \in A(t)}\left(\frac{1}{\eta} Q_{i}(t)+w_{i} u_{i}\right) \\ 
     \stackrel{(\rm a)}{\leq} & \sum_{i \in A^{\prime}(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} u_{i}\right)-\sum_{i \in A(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} u_{i}\right) \\ 
     \stackrel{(\rm b)}\leq & \sum_{i \in A^{\prime}(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} u_{i}\right)-\sum_{i \in A(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} u_{i}\right) \\ 
     +&\sum_{i \in A(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} \theta_{i}(t)\right) -\sum_{i \in A^{\prime}(t)}\left(\frac{1}{\eta}Q_{i}(t)+ w_{i} \theta_{i}(t)\right) \\
     =& {\sum_{i \in A(t)} w_{i}\left(\theta_{i}(t)-u_{i}\right)} + {\sum_{i \in A^{\prime}(t)} w_{i}\left(u_{i}-\theta_{i}(t)\right)},
     \end{aligned}
\end{equation}
where (a) is due to the definition of $A^\prime(t)$ in (\ref{eq:1eeeeee}) and (b) is due to (\ref{eq:1eee}).

Substituting (\ref{eq:ct}) into (\ref{eq:regretbound}) concludes the proof.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma  \ref{lm:ft}}
\begin{proof}
Let event $\mathcal{A}_i(t) := \left\{\hat{u}_i(t) - u_i \leq \gamma_i(t)\right\}$.

Then, we have $\Pr\left(\mathcal{J}_i(t)\right)$
\begin{equation}\label{eq:prnf}
\begin{aligned}
   =& \Pr\left({\mathcal{J}_i(t)}|\mathcal{A}_i(t) \right) \Pr(\mathcal{A}_i(t)) + \Pr\left({\mathcal{J}_i(t)}|\overline{\mathcal{A}_i(t)} \right) \Pr(\overline{\mathcal{A}_i(t)})\\
   \leq&\Pr\left({\mathcal{J}_i(t)}|\mathcal{A}_i(t)\right) + \Pr\left(\overline{\mathcal{A}_i(t)}\right).
\end{aligned}
\end{equation}

Let $\mathbf{F}_{\alpha,\beta}^{Beta}(\cdot)$ denote the CDF of Beta distribution with parameters $\alpha$ and $\beta$, and $\mathbf{F}_{n,p}^{B}(\cdot)$ denote the CDF of Binomial distribution with parameters $n$ and $p$.

With above notations, we can bound $\Pr\left({\mathcal{J}_i(t)}|\mathcal{A}_i(t)\right)$ as follows:
\begin{equation}\label{eq:pra1}
\begin{aligned}
    \Pr\left({\mathcal{J}_i(t)}|\mathcal{A}_i(t)\right) =& \Pr\left(\theta_i(t)>u_i+2\gamma_i(t)|\mathcal{A}_i(t)\right)\\
    \stackrel{(\rm a)}{\leq} & \Pr\left(\theta_i(t)>\hat{u}_i(t) + \gamma_i(t)\right)\\
    = & \mathbb{E}\left[{\Pr\left(\theta_i(t)>\hat{u}_i(t)  + \gamma_i(t) | \mathcal{F}_{t-1} \right)}\right],
\end{aligned}
\end{equation}
where (a) is due to the fact that $u_i + 2\gamma_i(t) \geq \hat{u}_i(t) + \gamma_i(t)$ conditioned on $\mathcal{A}_i(t)$ happens.

Since given $\mathcal{F}_{t-1}$, $\hat{u}_i(t)$ and $\gamma_i(t)$ are determined, we have
\begin{equation}\label{eq:pra3}
\begin{aligned}
     &\Pr\left(\theta_i(t)>\hat{u}_i(t) + \gamma_i(t) | \mathcal{F}_{t-1} \right)\\ 
    =& 1-\mathbf{F}_{\alpha_i(t),\beta_i(t)}^{Beta}\left(\hat{u}_i(t) + \gamma_i(t)\right)  \\
    \stackrel{(\rm b)}{=}& \mathbf{F}_{\alpha_i(t)+\beta_i(t)-1,\hat{u}_i(t)+\gamma_i(t)}^{B}\left(\alpha_i(t)-1\right), \\
\end{aligned}
\end{equation}
where (b) is due to Fact 3 in \cite{Agrawal2017} for the relationship between Beta and Binomial distributions. 

Define $d(a,b)$ as the KL divergence between $a$ and $b$. Since $\alpha_i(t)-1 = \hat{u}_i(t)(\alpha_i(t)+\beta_i(t)-2)$, (\ref{eq:pra3}) can be further bounded by

\begin{equation}\label{eq:pra2}
    \begin{aligned}
    &\mathbf{F}_{\alpha_i(t)+\beta_i(t)-1,\hat{u}_i(t)+\gamma_i(t)}^{B}\left(\hat{u}_i(t)(\alpha_i(t)+\beta_i(t)-1)\right) \\
    \stackrel{(\rm a)}{\leq} & e^{-(\alpha_i(t)+\beta_i(t)-1)d(\hat{u}_i(t), \hat{u}_i(t)+\gamma_i(t))}\\
    \stackrel{(\rm b)}{\leq} & e^{-h_i(t)\frac{|\hat{u}_i(t)-\hat{u}_i(t)-\gamma_i(t)|^2}{2}}\\
    =& e^{-h_i(t)\frac{\gamma^2_i(t)}{2}}\\
    =& \frac{1}{T},
    \end{aligned}
\end{equation}
where (a) is due to Fact 1 in \cite{Agrawal2017} by the Chernoff-Hoeffding bound and (b) is due to the fact that $d(a,b)\geq \frac{|a-b|^2}{2}$.
Substituting (\ref{eq:pra2}) and (\ref{eq:pra3}) into (\ref{eq:pra1}), we have
\begin{equation}\label{eq:pra4}
\begin{aligned}
    \Pr\left({\mathcal{J}_i(t)}|\mathcal{A}_i(t)\right)\leq \frac{1}{T}.
\end{aligned}
\end{equation}

On the other hand, $\Pr\left(\overline{\mathcal{A}_i(t)}\right)$ can be written as
\begin{equation*}\label{eq:prna1}
    \Pr\left(\overline{\mathcal{A}_i(t)}\right) = \mathbb{E}\left[\Pr\left(\overline{\mathcal{A}_i(t)} | \mathcal{F}_{t-1}\right)\right].
\end{equation*}
Given $\mathcal{F}_{t-1}$,  $\hat{u}_i(t)$ and $\gamma_i(t)$ are determined. Then also by Chernoff-Hoeffding inequality (Fact 2 in \cite{Agrawal2017}), we have
\begin{equation*}\label{eq:prna}
    \begin{aligned}
        \Pr\left(\overline{\mathcal{A}_i(t)}| \mathcal{F}_{t-1}\right) =& \Pr(\hat{u}_i(t) - u_i > \gamma_i(t))\\
        \leq& e^{-2 (\gamma_i(t))^2h_i(t)}=\frac{1}{T^4}.
    \end{aligned}
\end{equation*}
Therefore,  we have
\begin{equation}\label{eq:prna3}
    \Pr\left(\overline{\mathcal{A}_i(t)}\right) \leq \frac{1}{T^4}
\end{equation}

Substituting (\ref{eq:prna3}), (\ref{eq:pra4}) into (\ref{eq:prnf}) concludes the proof.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma \ref{lm:kt}}
\begin{proof}
Define event $\mathcal{G}_i(t)$ as
\begin{equation*}
    \mathcal{G}_i(t) := \{u_i-\hat{u}_i(t) \leq \varepsilon_i(t)\}.
\end{equation*}
We can decompose $\Pr\left({\mathcal{K}_i(t)}\right)$ as follows
\begin{equation}\label{eq:prnk}
\begin{aligned}
    &\Pr\left({\mathcal{K}_i(t)}|\mathcal{G}_i(t) \right) \Pr(\mathcal{G}_i(t)) + \Pr\left({\mathcal{K}_i(t)}|\overline{\mathcal{G}_i(t)} \right) \Pr(\overline{\mathcal{G}_i(t)})\\
   \leq&\Pr\left({\mathcal{K}_i(t)}|\mathcal{G}_i(t)\right) + \Pr\left(\overline{\mathcal{G}_i(t)}\right).
\end{aligned}
\end{equation}
For each arm $i$, since $u_i-2\varepsilon_i(t)\leq \hat{u}_i(t)-{\varepsilon_i(t)}$ when $\mathcal{G}_i(t)$ happens, we have $\Pr\left(\theta_i(t)<u_i-2\varepsilon_i(t)|\mathcal{G}_i(t)\right)$ bounded by
\begin{equation}\label{eq:pr1}
\begin{aligned}
     & \Pr\left(\theta_i(t)<\hat{u}_i-\varepsilon_i(t)\right)=  \mathbb{E}\left[\Pr\left(\theta_i(t)<\hat{u}_i-\varepsilon_i(t) | \mathcal{F}_{t-1}  \right) \right]
\end{aligned}
\end{equation}
Given $\mathcal{F}_{t-1}$, $\hat{u}_i(t)$ and $\varepsilon_i(t)$ are determined. Then, we can write $\Pr\left(\theta_i(t)<\hat{u}_i(t)-\varepsilon_i(t) | \mathcal{F}_{t-1}\right)$ as
\begin{equation}\label{eq:pr11}
\begin{aligned}
     &\mathbf{F}_{\alpha_i(t), \beta_i(t)}^{Beta}(\hat{u}_i(t)-{\varepsilon_i(t)})\\
     = & 1 -  \mathbf{F}_{\alpha_i(t) + \beta_i(t)-1, \hat{u}_i(t)-{\varepsilon_i(t)}}^{B}(\alpha_i(t)-1) \\
      \stackrel{(\rm b)} {=} & 1 -  \mathbf{F}_{h_i(t) + 1, \hat{u}_i(t)-{\varepsilon_i(t)}}^{B}(\hat{u}_i(t) h_i(t)),
\end{aligned}
\end{equation}
where  (b) is due to $h_i(t) = \alpha_i(t) + \beta_i(t)-2$ and $\alpha_i(t)-1 = \hat{u}_i(t)h_i(t)$.

%Next, we prove $\mathbf{F}_{h_i(t) + 1, \hat{u}_i-{\varepsilon_i(t)}}^{B}(\hat{u}_i h_i(t))$ is lower bounded. 
Let $Y_{j}$ be an outcome of the $j$-th Bernoulli trial with mean value $\hat{u}_i(t)-{\varepsilon_i(t)}$. $S_i := \sum\limits_{j=1}^{h_i(t)+1} Y_j$ is a random variable generated from Binomial distribution with parameters $h_i(t) + 1$~(number of trials) and $\hat{u}_i(t)-{\varepsilon_i(t)}$~(mean value). Then, we have
\begin{equation}\label{eq:Fb1m}
\begin{aligned}
    F_{h_i(t) + 1, \hat{u}_i(t)-{\varepsilon_i(t)}}^{B}(\hat{u}_i(t) h_i(t)) =& \Pr\left(S_i \leq \hat{u}_i(t) h_i(t)\right) \\
    = & 1 - \Pr\left(S_i > \hat{u}_i(t) h_i(t)\right).
\end{aligned}
\end{equation}
Substituting (\ref{eq:Fb1m}) into (\ref{eq:pr11}), we have
\begin{equation}\label{eq:fb2m}
    \mathbf{F}_{\alpha_i(t), \beta_i(t)}^{Beta}(\hat{u}_i(t)-{\varepsilon_i(t)})=\Pr\left(S_i > \hat{u}_i h_i(t)\right).
\end{equation}
We can rewrite $\Pr\left(S_i > \hat{u}_i h_i(t)\right)$ as
\begin{equation*}\label{eq:lema22}
\begin{aligned}
\Pr\left(S_i > n \mathbb{E}[Y_j]+\delta_i\right),
\end{aligned}
\end{equation*}
where $n=h_i(t)+1$, $\mathbb{E}[Y_j]=\hat{u}_i(t)-{\varepsilon_i(t)}$, and $\delta_i = \hat{u}_i(t) h_i(t)-(\hat{u}_i(t)-{\varepsilon_i(t)})(h_i(t)+1)$.

Therefore, according to the Chernoff–Hoeffding bound (Fact 2 in \cite{Agrawal2017}), we have 
\begin{equation*}
\begin{aligned}
    &\Pr\left(S_i > \hat{u}_i(t) h_i(t)\right)\\
    \leq& e^{-2(\delta_i)^2/n^2}\\
    =&e^{-2 \left(\hat{u}_i(t) h_i(t) - (\hat{u}_i(t)-{\varepsilon_i(t)})(h_i(t)+1)\right)^2/(h_i(t)+1)}\\
    =& e^{-2(\hat{u}^2_i(t) -  2 \hat{u}_i(t) \varepsilon_i(t)  (h_i(t)+1) + {\varepsilon_i(t)^2}(h_i(t)+1)^2)/(h_i(t)+1)} \\
    \leq & e^{-2( -  2 \hat{u}_i(t) \varepsilon_i(t) + {\varepsilon_i(t)^2}(h_i(t)+1))}\\
    = & e^{4 \hat{u}_i(t) \varepsilon_i(t) -2{\varepsilon_i(t)^2}(h_i(t)+1)}\\
    \leq & e^{4 \varepsilon_i(t) -2{\varepsilon_i(t)^2}h_i(t)}.
\end{aligned}
\end{equation*}
When  $h_i(t) \geq 4$, we have $h_i(t) \geq \frac{8}{\ln t}$, which means $4 \varepsilon_i(t) \leq \varepsilon^2_i(t)h_i(t)$. Then,
\begin{equation}\label{eq:g1}
\begin{aligned}
    \Pr\left(S_i > \hat{u}_i(t) h_i(t)\right) \leq e^{4 \varepsilon_i(t) -2{\varepsilon_i(t)^2}h_i(t)} \leq e^{-{\varepsilon_i^2(t)}h_i(t)}  = \frac{1}{t^2}.
\end{aligned}    
\end{equation}
Substituting (\ref{eq:g1}) into (\ref{eq:fb2m}), we have
\begin{equation*}
    \Pr\left(\theta_i(t)<\hat{u}_i(t)-\varepsilon_i(t) | \mathcal{F}_{t-1}  \right) \leq \frac{1}{t^2}.
\end{equation*}
Therefore,
\begin{equation*}\label{eq:t22}
    \Pr\left(\theta_i(t)<\hat{u}_i(t)-\varepsilon_i(t)\right) \leq \mathbb{E}\left[\Pr\left(\theta_i(t)<\hat{u}_i(t)-\varepsilon_i(t) | \mathcal{F}_{t-1}  \right) \right] = \frac{1}{t^2}.
\end{equation*}
On the other hand, $\Pr \left( \overline{\mathcal{G}_i(t)} \right) = \mathbb{E}\left[\Pr \left( \overline{\mathcal{G}_i(t)} | \mathcal{F}_{t-1} \right) \right]$. Given $\mathcal{F}_{t-1}$, $\hat{u}_i(t)$ and $\epsilon_i(t)$ is determined, and $\Pr \left( \overline{\mathcal{G}_i(t)} | \mathcal{F}_{t-1} \right)$ can be bounded by the Chernoff–Hoeffding bound (Fact 2 in \cite{Agrawal2017}) :
\begin{equation*}
\begin{aligned}
    \Pr \left( \overline{\mathcal{G}_i(t)}| \mathcal{F}_{t-1} = F_{t-1} \right)=& \Pr \left(\hat{u}_i(t) \leq u_i - {\varepsilon_i(t)} | \mathcal{F}_{t-1} = F_{t-1} \right)\\
    \leq & e^{-2 ({\varepsilon_i(t)})^2 h_i(t)}\\
    =& \frac{1}{t^4}.
\end{aligned}
\end{equation*}
Therefore, $\Pr \left( \overline{\mathcal{G}_i(t)} \right)$ can be bounded by $\frac{1}{t^4}$
\end{proof}


\subsubsection{Proof of Lemma \ref{lm:gs}}
\begin{proof}
Let event $\mathcal{C}_i(t)$ be defined as
\begin{equation*}
    \mathcal{C}_i(t) := \left\{\hat{u}_i(t) - u_i \leq \gamma_i(t)\right\}.
\end{equation*}
Then, $\Pr\left({\mathcal{J}_i(t)}\right)$ can be written as
\begin{equation}\label{eq:prnh}
\begin{aligned}
   &\Pr\left({\mathcal{J}_i(t)}|\mathcal{C}_i(t) \right) \Pr(\mathcal{C}_i(t)) + \Pr\left({\mathcal{J}_i(t)}|\overline{\mathcal{C}_i(t)} \right) \Pr(\overline{\mathcal{C}_i(t)})\\
   \leq&\Pr\left({\mathcal{J}_i(t)}|\mathcal{C}_i(t)\right) + \Pr\left(\overline{\mathcal{C}_i(t)}\right).
\end{aligned}
\end{equation}
Since  $u_i + 2\gamma_i(t) \geq \hat{u}_i(t) + \gamma_i(t)$ when $\mathcal{C}_i(t)$ happens, $\Pr\left({\mathcal{J}_i(t)}|\mathcal{C}_i(t)\right)$ can be bounded by
\begin{equation*}
\begin{aligned}
    &\Pr\left(\theta_i(t) > \hat{u}_i(t) + \gamma_i(t)\right)\\
    =& \mathbb{E}\left[\Pr\left(\theta_i(t) > \hat{u}_i(t) + \gamma_i(t) | \mathcal{F}_{t-1}\right)\right].
\end{aligned}
\end{equation*}
Given $\mathcal{F}_{t-1}$, $\hat{u}_i(t)$ and $\gamma_i(t)$ are determined. Then according to Fact 4 in \cite{Agrawal2017} for the concentration of Gaussian distributions, we have
\begin{equation*}
\begin{aligned}
    \Pr\left(\theta_i(t) > \hat{u}_i(t) + \gamma_i(t) | \mathcal{F}_{t-1}\right)
    \leq& \frac{1}{2} e^{-(\gamma_i(t)\cdot (h_i(t)+1))^2/2}\\
    \leq& \frac{1}{2} e^{-(\gamma_i(t)\cdot (h_i(t)))^2/2}\\
    =& \frac{1}{2}  \frac{1}{T^{h_i(t)}}\\
    \leq& \frac{1}{T}.
\end{aligned}
\end{equation*}
where the last inequality is due to the condition $h_i(t) > 0$.
Therefore, $\Pr\left({\mathcal{J}_i(t)}|\mathcal{C}_i(t)\right)$ can be bounded by $\frac{1}{T}$.

On the other hand, by the Chernoff–Hoeffding bound, we have
\begin{equation*}
    \Pr\left(\overline{\mathcal{C}_i(t)}\right) \leq \frac{1}{T^4},
\end{equation*}
Therefore, $\Pr\left({\mathcal{J}_i(t)}\right)$ can be bounded by $\frac{1}{T}+\frac{1}{T^4}$.

$\Pr\left(\overline{\mathcal{H}_i(t)}\right)$ can be bounded in the same way.
\end{proof}







==> Thompson Sampling for Combinatorial Semi-bandits with Sleeping Arms and Long-Term Fairness Constraints/7-Experiments.tex <==




% \begin{figure*}\label{fig:fairness}
% \subfloat [OPT on arm $1$] {\label{fig:fairness:a}
% \epsfig{file=Figures/result_syn_1_Selectfraction_OPT_arm1.eps, width = 0.66\columnwidth}
% }
% \subfloat [OPT on arm $2$] {\label{fig:fairness:b}
% \epsfig{file = Figures/result_syn_1_Selectfraction_OPT_arm2.eps, width = 0.66\columnwidth}
% }
% \subfloat [OPT on arm $3$] {\label{fig:fairness:c}
% \epsfig{file= Figures/result_syn_1_Selectfraction_OPT_arm3.eps, width = 0.66\columnwidth}
% }

% \subfloat [LFG on arm $1$] {\label{fig:fairness:d}
% \epsfig{file=Figures/result_syn_1_Selectfraction_LFG_arm1.eps, width = 0.66\columnwidth}
% }
% \subfloat [LFG on arm $2$] {\label{fig:fairness:e}
% \epsfig{file = Figures/result_syn_1_Selectfraction_LFG_arm2.eps, width = 0.66\columnwidth}
% }
% \subfloat [LFG on arm $3$] {\label{fig:fairness:f}
% \epsfig{file= Figures/result_syn_1_Selectfraction_LFG_arm3.eps, width = 0.66\columnwidth}
% }

% \subfloat [TSCSF-B on arm $1$] {\label{fig:fairness:g}
% \epsfig{file=Figures/result_syn_1_Selectfraction_TS_B_arm1.eps, width = 0.66\columnwidth}
% }
% \subfloat [TSCSF-B on arm $2$] {\label{fig:fairness:h}
% \epsfig{file=Figures/result_syn_1_Selectfraction_TS_B_arm2.eps, width = 0.66\columnwidth}
% }
% \subfloat [TSCSF-B on arm $3$] {\label{fig:fairness:i}
% \epsfig{file=Figures/result_syn_1_Selectfraction_TS_B_arm3.eps, width = 0.66\columnwidth}
% }
% \caption{Fairness of each arm for the first setting}\label{sec:fairness}
% \vspace{-13pt}
% \end{figure*}

\section{Evaluations and Applications}\label{sec:evaluation}

\subsection{Numerical Experiments}
In this section, we compare the TSCSF-B algorithm with the LFG algorithm~\cite{li2019combinatorial} in two settings. The first setting is identical to the setting in~\cite{li2019combinatorial},  where $N=3$, $m=2$, and $w_i = 1, \forall i \in \mathcal{N}$. The mean reward vector for the three arms is $(0.4, 0.5, 0.7)$. The availability of the three arms is $(0.9,0.8,0.7)$, and the fairness constraints for the three arms are $(0.5,0.6,0.4)$. To see the impact of $\eta$ on the time-averaged regret and fairness constraints, we compare the algorithms under $\eta=1, 10, 1000$ and $\infty$ in a time horizon $T = 2 \times 10^4$, where $\eta \rightarrow \infty$ indicates that both algorithms do not consider the long-term fairness constraints.

Further, we test the algorithms in a more complicated setting where $N=6$, $m=3$, and $w_i = 1, \forall i \in \mathcal{N}$. The mean reward vector for the six arms is $(0.52,0.51,0.49,0.48,0.7,0.8)$. The availability of the six arms is $(0.7,0.6,0.7,0.8,0.7,0.6)$, and the fairness constraints for the six arms are $(0.4,0.45,0.3,0.45,0.3,0.4)$.
This setting is challenging because higher fairness constraints are given to the arms with less mean rewards and the arms with lower availability (i.e., arms $2$ and $4$).
According to Corollary \ref{cr:1}, we set $\eta=\sqrt{\frac{NT}{m\ln T}} = 63.55$
%100\sqrt{\frac{NT}{m\ln T}}=6355$
and $\infty$, and $T = 2 \times 10^4$.
Note that the following results are the average of $100$ independent experiments. We omit the plotting of confidence interval and deviations because they are too small to be seen from the figures and are also omitted in most bandit papers.

\subsubsection{Time-Averaged Regret}
The time-averaged regret results under the first setting and the second setting are shown in Fig.~\ref{fig:3regret} and Fig.~\ref{fig:setting2}, respectively.
\begin{figure}[h]
\subfloat [$\eta = 1$] {\label{fig:3regret:a}
\epsfig{file=Figures/result_syn_1_regret_eta_1, width = 0.48\columnwidth}
}
\subfloat [$\eta = 10$] {\label{fig:3regret:b}
\epsfig{file = Figures/result_syn_1_regret_eta_10, width = 0.48\columnwidth}
}

% \subfloat [$\eta = 100$] {\label{fig:3regret:c}
% \epsfig{file= Figures/result_syn_1_regret_eta_100.eps, width = 0.48\columnwidth}
% }
\subfloat [$\eta = 1000$] {\label{fig:3regret:d}
\epsfig{file = Figures/result_syn_1_regret_eta_1000, width = 0.48\columnwidth}
}
\subfloat [$\eta \rightarrow \infty $] {\label{fig:3regret:e}
\epsfig{file = Figures/result_syn_1_regret_eta_0, width = 0.48\columnwidth}
}
\caption{Time-averaged regret for the first setting.}\label{fig:3regret}
\vspace{-13pt}
\end{figure}


\begin{figure}
\subfloat [$\eta = \sqrt{\frac{NT}{m\ln T}}$] {\label{fig:setting2:a}
\epsfig{file=Figures/result_syn_2_regret_eta_1, width = 0.48\columnwidth}
}
% \subfloat [$\eta = 100\sqrt{\frac{NT}{m\ln T}}$] {\label{fig:setting2:b}
% \epsfig{file = Figures/result_syn_2_regret_eta_100.eps, width = 0.48\columnwidth}
% }
\subfloat [$\eta \rightarrow \infty $] {\label{fig:setting2:c}
\epsfig{file= Figures/result_syn_2_regret_eta_0, width = 0.48\columnwidth}
}

\caption{Time-averaged regret for the second setting.}\label{fig:setting2}
\vspace{-13pt}
\end{figure}
In each subplot, the $x$-axis represents the rounds and the $y$-axis is the time-averaged regret. A small figure inside each subplot zooms in the first $100$ rounds. We also plot the \emph{OPT with considering fairness~(Opt-F)} (i.e., the optimal solution to CSMAB-F), and \emph{OPT without considering fairness~(Opt-NF)} (i.e., the optimal solution to CSMAB). The time-averaged regret of Opt-NF is always below Opt-F, since Opt-NF does not need to satisfy the fairness constraints and can always achieve the highest rewards. By definition, the regret of Opt-F is always $0$.

We can see that the proposed TSCSF-B algorithm has a better performance than the LFG algorithm, since it converges faster, and achieves a lower regret, as shown in Fig.~\ref{fig:3regret} and Fig.~\ref{fig:setting2}. It is noteworthy that the gap between TSCSF-B and LFG is larger in Fig.~\ref{fig:setting2}, which indicates that TSCSF-B performs better than LFG in more complicated scenarios.

In terms of $\eta$, the algorithms with a higher $\eta$ can achieve a lower time-averaged regret. For example, in the first setting, the lowest regrets achieved by the two considered algorithms are around $0.03$ when $\eta = 1$,  but they are much closer to Opt-F when $\eta = 10$. However, when we continue to increase $\eta$ to $1000$ (see Fig.~\ref{fig:3regret:d}), the considered algorithms achieve a negative time-averaged regret around $0.2 \times 10^4$ rounds, but recover to the positive value afterwards. This is due to the fact that with a high $\eta$ the algorithms preferentially pull arms with the highest mean rewards, but the queues still ensure the fairness can be achieved in future rounds.
When $\eta \rightarrow \infty$ (see Fig.~\ref{fig:3regret:e} and Fig.~\ref{fig:setting2:c}), the fairness constraints are totally ignored and the regrets of the considered algorithms converge to Opt-NF. Therefore, $\eta$ significantly determines whether the algorithms can satisfy and how quickly they satisfy the fairness constraints.

% We note that the reason why the gap between TSCSF-B and LFG is small in Fig.~\ref{fig:3regret} is that the testing setting is too simple (only $3$ arms). We have tested that when the number of arms increases, the gap becomes clearer.
%Although the algorithms in (d) achieves more rewards than Opt-F, the fairness constraints are sacrificed, as inferred in Fig.~. The reason for this phenomenon is that a higher $\eta$ means we consider less fairness but more on the rewards, as discussed in Sec.~\ref{sec:fairness}.

%The results of the second setting are shown in Fig.~\ref{fig:setting2}. We can see that in the more complicated setting, the superiority of our algorithms is more obvious. The regret gap between the proposed algorithms and the LFG algorithm becomes larger than that in the first setting when $\eta \rightarrow \infty$, as shown in Fig.~\ref{fig:setting2:c}.
%Additionally, when we set $\eta$ to be proportional of $\sqrt{\frac{NT}{m \ln T}}$, the regret gap between the considered algorithms and Opt-F is much tighter, as shown in Fig.~\ref{fig:setting2:a} and Fig.~\ref{fig:setting2:b}. Especially in Fig.~\ref{fig:setting2:b}, we can observe that the considered algorithms converge to the almost same value as Opt-F.

%Regarding the proposed algorithms, TSCSF-B has a better performance than TSCSF-G in both settings. Take Fig.~\ref{fig:3regret:a} for example, although they have similar time-averaged regrets in the end, TSCSF-B has a lower regret in the first several rounds. This may due to the posterior samples from Gaussian distribution have a wide range, while the samples from Beta distribution are limited in $[0,1]$.

\subsubsection{Fairness Constraints}





% \begin{figure}[h]
% \subfloat [TSCSF-B] {\label{fig:tightness:a}
% \epsfig{file= Figures/result_syn_1_Selectfraction_TS_B_arm1.eps, width = 0.48\columnwidth}
% }
% \subfloat [LFG] {\label{fig:tightness:b}
% \epsfig{file= Figures/result_syn_1_Selectfraction_LFG_arm1.eps, width = 0.48\columnwidth}
% }

% % \subfloat [$\eta = 100$] {\label{fig:tightness:c}
% % \epsfig{file= Figures/result_syn_1_bound_eta_100.eps, width = 0.48\columnwidth}
% % }
% % \subfloat [$\eta \rightarrow \infty$] {\label{fig:tightness:c}
% % \epsfig{file= Figures/result_syn_1_bound_eta_Inf.eps, width = 0.48\columnwidth}
% % }
% \caption{Fairness of arm $1$ in the first setting.}\label{sec:fairness}
% \vspace{-13pt}
% \end{figure}


% \begin{figure}[h]
% \subfloat [LFG on arm $2$] {\label{fig:fairness2:a}
% \epsfig{file= Figures/result_syn_2_Selectfraction_LFG_arm2, width = 0.48\columnwidth}
% }
% \subfloat [LFG on arm $4$] {\label{fig:fairness2:b}
% \epsfig{file= Figures/result_syn_2_Selectfraction_LFG_arm4.eps, width = 0.48\columnwidth}
% }

% \subfloat [TSCSF-B on arm $2$] {\label{fig:fairness2:c}
% \epsfig{file= Figures/result_syn_2_Selectfraction_TS_B_arm2.eps, width = 0.48\columnwidth}
% }
% \subfloat [TSCSF-B on arm $4$] {\label{fig:fairness2:c}
% \epsfig{file= Figures/result_syn_2_Selectfraction_TS_B_arm4.eps, width = 0.48\columnwidth}
% }
% \caption{Fairness of arms $2$ and $4$ in the second setting.}\label{sec:fairness2}
% \vspace{-13pt}
% \end{figure}

% \begin{figure}[h]
% \subfloat [TSCSF-B] {\label{fig:tightness:a}
% \epsfig{file= Figures/result_syn_1_final_selection_fraction.eps, width = 0.48\columnwidth}
% }
% \subfloat [LFG] {\label{fig:tightness:b}
% \epsfig{file=  Figures/result_syn_2_final_selection_fraction.eps, width = 0.48\columnwidth}
% }

% % \subfloat [$\eta = 100$] {\label{fig:tightness:c}
% % \epsfig{file= Figures/result_syn_1_bound_eta_100.eps, width = 0.48\columnwidth}
% % }
% % \subfloat [$\eta \rightarrow \infty$] {\label{fig:tightness:c}
% % \epsfig{file= Figures/result_syn_1_bound_eta_Inf.eps, width = 0.48\columnwidth}
% % }
% \caption{Fairness of arm $1$ in the first setting.}\label{sec:fairness}
% \vspace{-13pt}
% \end{figure}



In the first setting, we show in Fig.~\ref{fig:fairness1} the final satisfaction of fairness constraints for all  arms under $\eta = 1000$.  $\eta = 1000$ is an interesting setting where the fairness constraints are not satisfied in the first few rounds as aforementioned. We want to point out in the first setting, the fairness constraint for arm $1$ is relatively difficult to be satisfied, since arm $1$ has the lowest mean reward but has a relative high fairness constraint.  However,  we can see that the fairness constraints for all arms are satisfied finally, which means both TSCSF-B and LFG are able to ensure the fairness constraints in this simple setting.

In the second setting with $\eta = \sqrt{\frac{NT}{m\ln T}} = 63.55$, the fairness constraints for arms $2$ and $4$ are difficult to satisfy, as both arms have high fairness constraints but low availability or low mean reward. However, both TSCSF-B and LFG manage to satisfy the fairness constraints for all the $6$ arms, as shown in  Fig.~\ref{fig:fairness2}.
% We can see from Fig.~\ref{sec:fairness} that, Opt-NF cannot fulfill the fairness constraints and Opt-F just meets the constraints, which is expected since arm $1$ has the lowest mean reward.
% The results of TSCSF-B and LFG are similar, the fairness constraint is not fulfilled in the first few rounds, since both algorithms are taking less importance on the virtual queues when $\eta =1000$. However, TSCSF-B drops much lower than LFG as TSCSF-B pulls other arms with higher mean rew ards in the first few rounds. We argue that this does not mean LFG performs better than TSCSF-B, as we only focus on the long-term fairness constraints, and both algorithm meet this requirement well.

\begin{figure}[h]
    \centering
    \includegraphics[width = 0.8\columnwidth]{Figures/result_syn_1_final_selection_fraction}
    \caption{Satisfaction of fairness constraints in the first setting.}
    \label{fig:fairness1}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width = 0.8\columnwidth]{Figures/result_syn_2_final_selection_fraction}
    \caption{Satisfaction of fairness constraints in the second setting.}
    \label{fig:fairness2}
\end{figure}


%Next, we look into the satisfaction of fairness constraints in the second setting. For brevity, we only show the arms, of which the pull times by Opt-F just meet the fairness constraints, as shown in Fig.~\ref{sec:fairness2}. We can see that, when $\eta = \sqrt{\frac{NT}{m \ln T}}$, both algorithms converge fast to the optimal solution, while when $\eta = 100 \sqrt{\frac{NT}{m \ln T}}$, the speed of convergence is slower. From the trend, both algorithms are able to satisfy the fairness constraints. Compare Fig.~\ref{sec:fairness2} with Fig.~\ref{sec:fairness}, it can be found that $\eta = \sqrt{\frac{NT}{m \ln T}}$ is an appropriate value, which can help the algorithm converge to the optimal solution quickly.

\subsection{Tightness of the Upper bounds}
Finally, we show the tightness of our bounds in the second setting, as plotted in Fig.~\ref{fig:tightness}. The $x$-axis represents the change of the time horizon $T$, and the $y$-axis is the logarithmic time-averaged regret in the base of $e$.

We can see that, the upper bound of TSCSF-B is always below that of LFG. However, there is a big gap between the TSCSF-B upper bound and the actual time-averaged regret in the second setting. This is reasonable, since the upper bound is problem-independent, but it is still of interest to find tighter bound for CSMAB-F problems.
% \begin{figure}[h]
% % \subfloat [$\eta=1$] {\label{fig:fairness2:a}
% % \epsfig{file= Figures/result_syn_1_bound_eta_1, width = 0.66\columnwidth}
% % }

% \subfloat [$\eta=\sqrt{\frac{NT}{m\ln T}}$] {\label{fig:fairness2:b}
% \epsfig{file= Figures/result_syn_2_bound.eps, width = 0.66\columnwidth}
% }
% \caption{Tightness of the upper bounds for TSCSF-B}\label{fig:tightness}
% \vspace{-13pt}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/result_syn_2_bound}
    \caption{Tightness of the upper bounds for TSCSF-B}
    \label{fig:tightness}
\end{figure}
%As we can see, the upper bounds uniformly bound the time-averaged regret of TSCSF-B over any time horizon T. In addition, we can observe that $\eta$ has a significant impact on the tightness of the bounds. As $\eta$ increases, the gap between the bound and the regret of the algorithm reduces, as shown in Fig.  to Fig.~\ref{fig:tightness:c}. When $\eta$ is large enough, if we continue to increase $\eta$, the reduction on the gap is trivial.

\subsection{High-rating movie recommendation System}
In this part, we consider a high-rating movie recommendation system. The objective of the system is to recommend high-rating movies to users, but the ratings for the considered movies are unknown in advance. Thus, the system needs to learn the ratings of the movies while simultaneously recommending the high-rating ones to its users. Specifically, when each user comes, the movies that are relevant to the user's preference are available to be recommended. Then, the system recommends the user with a subset of the available movies subject.
After consuming the recommended movies, the user gives feedback to the system, which can be used to update the ratings of the movies to better serve the upcoming users. In order to acquire accurate ratings or to ensure the diversity of recommended movies, each movie should be recommended at least a number of times.

The above high-rating movie recommendation problem can be modeled as a CSMAB-F problem under three assumptions.
First, we take serving one user as a round by assuming the next user always comes after the current user finishes rating. This assumption can be easily relaxed by adopting \emph{the delayed feedback framework} with an additive penalty to the regret~\cite{joulani2013online}.
Second, the availability set of movies is stochastically generated according to an unknown distribution.
Last, given a movie, the ratings are i.i.d. over users with respect to an unknown distribution. The second and third assumptions are feasible, as it has been discovered that the user preference and ratings towards movies have a strong relationship to the Zipf distribution~\cite{Cha07I,gill07youtube}.

\subsubsection{Setup}
We implement TSCSF-B and LFG on \emph{MovieLens 20M Dataset}~\cite{harper2016movielens}, which includes $20$ million ratings to $27,000$ movies by $138,000$ users. This dataset contains both users’ movie ratings between $1$ and $5$ and genre categories for each movie. In order to compare the proposed TSCSF-B algorithm to the LFG algorithm, we select $N=5$ movies with different genres as the ground set of arms $\mathcal{N}$, which are Toy Story (1995) in the genre of Adventure, Braveheart (1995) in Action, Pulp Fiction (1994) in Comedy, Godfather, The (1972) in Crime,  and Alien (1979) in Horror.

Then, we count the total number of ratings on the selected $5$ genres and calculate occurrence of each selected genre among the $5$ genres as the availability of the corresponding selected movie. We note that the availability of the selected movies is only used by the OPT-F algorithm and is not used to determine the available set of movies in each round. During the simulation, when each user comes, the available set of movies is determined by whether the user has rated or not these movies in the dataset.

The ratings are scaled into $[0,1]$ to satisfy as the rewards. We choose $28,356$ users who have rated at least one of the selected $5$ movies as the number of rounds~(one round one user according to the first assumption) for the algorithms, and take their ratings as the rewards to the recommended movies.
When each user comes, the system will select no more than $m=2$ movies for recommendation and each movie shares the same weight, i.e., $w_i = 1, \forall i \in \mathcal{N}$, and the same fairness constraints. The fairness constraints are set as $\mathbf{k} = [0.3,0.3,0.3,0.3,0.3]$ such that (\ref{eq:question}) has a feasible solution.

We adopt such an implementation, including the determination of the available movie set, the same movie weights, and the same fairness constraints, to ensure that our simulation brings noise as little as possible to the MovieLens dataset.

\subsubsection{Results}
We first show whether the considered algorithms are able to achieve accurate ratings. The final ratings of selected movies by TSCSF-B and LFG under $\eta = \sqrt{\frac{NT}{m\ln T}}$ and  $\infty$ are shown in Fig.~\ref{fig:Movieratings}. The reason why we set $\eta = O(\sqrt{\frac{NT}{m\ln T}})$ is due to Corollary~\ref{cr:1}.
We can observe that the performance of TSCSF-B is better than that of LFG, since the ratings of TSCSF-B are much closer to the true average ratings, while the ratings acquired by UCB are higher than the true average ratings.

The final satisfaction for the fairness constraints of the selected movies is shown in Fig.~\ref{fig:fractionfinal}. Both TSCSF-B and LFG can satisfy the fairness constraints of the five movies under $\eta=\sqrt{\frac{NT}{m\ln T}}$.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width = 0.85\columnwidth]{Figures/result_syn_movie_ratings.eps}
%     \caption{The final ratings of selected movies.}
%     \label{fig:Movieratings}
% \end{figure}
\begin{figure}[h]
\subfloat [] {\label{fig:Movieratings}
\epsfig{file= Figures/result_syn_movie_ratings, width = 0.48\columnwidth}
}
\subfloat [] {\label{fig:fractionfinal}
\epsfig{file= Figures/result_syn_movie_selection_fraction, width = 0.48\columnwidth}
}
\caption{(a) The final ratings of selected movies. (b) The final satisfaction for the fairness constraints of selected movies.}
\vspace{-13pt}
\end{figure}



On the other hand, the time-averaged regret is shown in Fig.~\ref{sec:movieregret}. We can see that the time-averaged regret of TSCSF-B is below that of LFG, which indicates the proposed TSCSF-B algorithm converges much faster. Since we are unable to obtain the true distribution of the available movie set~(as discussed in \emph{Setup}), the rewards achieved by the OPT-F algorithm may not be the optimal one, which explains why the lines of both TSCSF-B and LFG are below that of OPT-F in Fig.~\ref{sec:movieregret}.


Generally,  TSCSF-B performs much better than LFG in this application, which achieves better final ratings and a quicker convergence speed.

% \begin{figure}[h]
% \subfloat [$\eta=\sqrt{\frac{NT}{m\ln T}}$] {\label{fig:movieregret:a}
% \epsfig{file= Figures/result_syn_movie_regret_eta_1.eps, width = 0.48\columnwidth}
% }
% % \subfloat [$\eta=100\sqrt{\frac{NT}{m\ln T}}$] {\label{fig:movieregret:b}
% % \epsfig{file= Figures/result_syn_movie_regret_eta_100.eps, width = 0.48\columnwidth}
% % }
% \caption{Time-averaged regret bounds for the high-rating movie recommendation system.}\label{sec:movieregret}
% \vspace{-13pt}
% \end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width = 0.8\columnwidth]{Figures/result_syn_movie_regret_eta_1}
    \caption{Time-averaged regret bounds for the high-rating movie recommendation system.}
    \label{sec:movieregret}
\end{figure}




% Then, we show the fairness constraints of movies ``Toy Story'' and ``Braveheart''. We do not show the TSCSF-G algorithms since it has similar behaviour to TSCSF-B, and the fairness constraints for movies ``Toy Story'' and ``Braveheart'' are not easy to satisfy, since they do not have high rewards. As can be seen from Fig.~\ref{sec:fairnessMovie}, both LFG and TSCSF-B can successfully meet the fairness constraints when $\eta = \sqrt{\frac{NT}{m\ln T}}$, which achieve a comparable performance with OPT. When $\eta = 100 \sqrt{\frac{NT}{m\ln T}}$, both the algorithms do not satisfy the requirements at beginning, but show a tendency to converge to the required fairness constraints.



% \begin{figure}[h]
% \subfloat [Movie ``Toy Story'' with LFG] {\label{fig:fairness2:a}
% \epsfig{file= Figures/result_syn_movie_Selectfraction_LFG_arm1.eps, width = 0.48\columnwidth}
% }
% \subfloat [Movie ``Braveheart'' with LFG] {\label{fig:fairness2:b}
% \epsfig{file= Figures/result_syn_movie_Selectfraction_LFG_arm2.eps, width = 0.48\columnwidth}
% }

% \subfloat [Movie ``Toy Story'' with TSCSF-B] {\label{fig:fairness2:c}
% \epsfig{file= Figures/result_syn_movie_Selectfraction_TS_B_arm1.eps, width = 0.48\columnwidth}
% }
% \subfloat [Movie ``Braveheart'' with TSCSF-B] {\label{fig:fairness2:c}
% \epsfig{file= Figures/result_syn_movie_Selectfraction_TS_B_arm2.eps, width = 0.48\columnwidth}
% }
% \caption{Fairness of movies ``Toy Story'' and ``Braveheart''}\label{sec:fairnessMovie}
% \vspace{-13pt}
% \end{figure}


==> Thompson Sampling for Combinatorial Semi-bandits with Sleeping Arms and Long-Term Fairness Constraints/8-Conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this paper, we studied the stochastic combinatorial sleeping multi-armed bandit problem with fairness constraints, and designed the TSCSF-B algorithm with a provable problem-independent bound of $\widetilde{O}\left(\frac{\sqrt{mNT}}{T}\right)$ when $T \geq N$. Both the numerical experiments and real-world applications were conducted to verify the performance of the proposed algorithms.

As part of the future work, we would like to derive more rigorous relationship between $\eta$ and $T$ such that the algorithm can always satisfy the fairness constraints and achieves high rewards given any $T$, as well as tighter bounds.
